On the Alignment of Group Fairness with Attribute Privacy

Group fairness and privacy are fundamental aspects in designing trustworthy machine learning models. Previous research has highlighted conflicts between group fairness and different privacy notions. We are the first to demonstrate the alignment of group fairness with the specific privacy notion of attribute privacy in a blackbox setting. Attribute privacy, quantified by the resistance to attribute inference attacks (AIAs), requires indistinguishability in the target model's output predictions. Group fairness guarantees this thereby mitigating AIAs and achieving attribute privacy. To demonstrate this, we first introduce AdaptAIA, an enhancement of existing AIAs, tailored for real-world datasets with class imbalances in sensitive attributes. Through theoretical and extensive empirical analyses, we demonstrate the efficacy of two standard group fairness algorithms (i.e., adversarial debiasing and exponentiated gradient descent) against AdaptAIA. Additionally, since using group fairness results in attribute privacy, it acts as a defense against AIAs, which is currently lacking. Overall, we show that group fairness aligns with attribute privacy at no additional cost other than the already existing trade-off with model utility.

==> New/misc/4.2approachdef.tex <==
\section{Attribute Privacy via Fairness}\label{sec:approachdef}



We motivate the use of algorithmic fairness to mitigate \aia{s}. We then describe the theoretical results evaluating the effectiveness of \egd with \demparity and \eo as a defence against \adaptiveAIA. We also show in the Appendix~\ref{app:dp} that Differential Privacy (DP) in the context of machine learning gives no guarantee of protection against attribute privacy.


\noindent\textbf{\underline{Motivation}} Attribute privacy, i.e., resistance against \aia{s} requires $\targetmodel$'s predictions indistinguishable for different values of $S(\omega)$. Fairness algorithms such as \advdebias achieve this empirically where $\targetmodel$ is trained to output indistinguishable predictions (soft labels) for sensitive attributes. \egd, on the other hand, adds an additional constraint during training to ensure indistinguishable predictions (hard labels). Hence, we conjecture algorithmic fairness to act as a defence against \aia. In other words, training for fairness can help achieve attribute privacy due to their \textit{aligned} objectives.


\noindent\textbf{\underline{Mitigating \adaptiveAIASoft with \advdebias}} On training a model with \advdebias, we expect the model predictions (soft labels) to be indistinguishable compared to the case when model is trained without \advdebias (i.e., Figure~\ref{fig:distribution}). We present similar plots after training $\targetmodel$ with \advdebias in Figure~\ref{}. We find that in all the cases, the prediction distribution for different values of sensitive attributes are indistinguishable. Hence, we expect that an \adv with access to soft labels from $\targetmodel$ should not be able to infer $S(\omega)$. We empirically verify this in Section~\ref{}


\noindent\textbf{\underline{Mitigating \adaptiveAIAHard with \egd}} Recall that $\targetmodel$ can be trained with \egd to satisfy either \demparity or \eo. Different fairness definitions give different guarantees on mitigating \aia{s}. We theoretically evaluate the balanced \aia accuracy under both \demparity and \eo fairness constraints.


\begin{theorem}
\label{th:dpgood}
%If $\hat{Y}$ satisfies \demparity for $S$ then 
%for all attack model $\attackmodel:[0,1]\rightarrow[0,1]$ and for all threshold $\upsilon\in[0,1]$,
%the balanced \aia accuracy of~$\hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y}$ is equal to $\frac{1}{2}$
The maximum balanced \aia accuracy achievable is equal to $\frac{1}{2}(1+\text{dp-level of the $\targetmodel$})$ . 
\end{theorem}

\begin{proof}
We have seen in section \ref{sec:atthard} that the set $B$ of function from $\{0,1\}$ to $\{0,1\}$ contains four elements $b_0$, $b_1$, $b_2$ and $b,3$.
For every $b\in B$ the balanced \aia accuracy is 
$BA(b) = \frac{1}{2}(P(b\circ \hat{Y}=0|S=0) + P(b\circ \hat{Y}=1|S=1))$.
We have $BA(b_0) = BA(b_3) = \frac{1}{2}$ hence we can discard those elements when solving the attack optimisation problem.
This problem writes $\text{max}_{b\in B}B(A(b)) = \text{max}(BA(b_1), BA(b_2))$.
We remark that $b_1\circ \hat{Y}=\hat{Y}$ and $b_2\circ \hat{Y}=1 - \hat{Y}$.
Hence,
{\footnotesize
\begin{align*}
    BA(b_1) &= \frac{1}{2}(P(\hat{Y}=0|S=0) + P(\hat{Y}=1|S=1))\\
    &=\frac{1}{2}(1+P(\hat{Y}=1|S=1) - P(\hat{Y}=1|S=0))
\end{align*}
}
And
{\footnotesize
\begin{align*}
    BA(b_2)=\frac{1}{2}(1+P(\hat{Y}=1|S=0) - P(\hat{Y}=1|S=1))
\end{align*}
}
Thus,
{\footnotesize
\begin{align*}
    &\text{max}_{b\in B}BA(b) \\
    = &\frac{1}{2}\left(1+\text{max}\left(
    \begin{matrix}
        P(\hat{Y}=0|S=0) -P(\hat{Y}=1|S=1)\\ 
        P(\hat{Y}=1|S=0) -P(\hat{Y}=0|S=1)
    \end{matrix}
    \right)\right)\\
    =&\frac{1}{2}(1+|P(\hat{Y}=1|S=1) - P(\hat{Y}=1|S=0)|)
\end{align*}
}
%Let $\hat{Y}:\Omega\rightarrow\{0,1\}$ be a random variable that satisfies \demparity for $S$ and $\hat{S}$ be the inferred sensitive attribute from the attack classifier on exploiting $\hat{Y}$. Then,
%\begin{equation}
%\label{eq:defShat}
%    \hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y},
%\end{equation}
%where $\upsilon\in[0,1]$ and $\attackmodel:\{0,1\}\rightarrow[0,1]$ is a measurable function.

%We compute the balanced \aia accuracy to infer $\hat{S}$, given by, $\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))$.
%In this expression, we substitute the definition of $\hat{S}$ from Equation~\ref{eq:defShat} which gives us the conditional law of $Y$ knowing $S$.
%Using the Definition~\ref{def:dp}, we can compute the balanced \aia accuracy when training with \demparity.
%{
%\footnotesize
%\begin{align*}
%    &\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))\\
%    =&\frac{1}{2}(P({1_{[\upsilon,1]}\circ \attackmodel\circ\hat{Y}=1|S=1}) + %P({1_{[0,\upsilon]}\circ \attackmodel\circ\hat{Y}=0|S=0}))\\
%    =&\frac{1}{2}(P({\hat{Y}\in \attackmodel^{-1}([\upsilon,1])|S=1}) + P({\hat{Y}\in %\attackmodel^{-1}([0,\upsilon])|S=0})\\
%    =&\frac{1}{2}(1-P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})+P({\hat{Y}\in %\attackmodel^{-1}([0,\upsilon])|S=0})\\
%    =&\frac{1}{2}(1-P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})+P({\hat{Y}\in %\attackmodel^{-1}([0,\upsilon])|S=0})\\
%    =&\frac{1}{2}
%\end{align*}
%}
\end{proof}
In summary, satisfying \demparity indicates that the dp-level is zero, consequently, \textbf{if $\targetmodel$ satisfies \demparity then no $\attackmodel$ will perform better than a random guess}. Hence, \demparity can ensure the confidentiality of $S(\omega)$.
We now present the balanced \aia accuracy under \eo constraint.

\begin{theorem}
\label{th:eoo}
If $\hat{Y}$ satisfies \eo for $Y$ and $S$ then for all attack model $\attackmodel:[0,1]\rightarrow[0,1]$ and for all threshold $\upsilon\in[0,1]$, the balanced \aia accuracy of $\hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y}$ is greater than $\frac{1}{2}$. In addition, balanced \aia accuracy is random guess $\frac{1}{2}$ if and only if $Y$ is independent of $S$ or $\hat{Y}$ is independent of $Y$.
\end{theorem}

\begin{proof}
    Let $\hat{Y}:\Omega\rightarrow\{0,1\}$ a random variables classifier of $Y$ that satisfies \eo for $S$.
    Let $\hat{S}$ an attack classifier of $S$ using $\hat{Y}$ with the same definition as in equation \ref{eq:defShat}.
    For this proof, we use the total probability law to make use of the conditional law of $\hat{Y}$ knowing $(S,Y)$.
    {
    \footnotesize
    \begin{align}
         &\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))\\
        =&\frac{1}{2}(P({1_{[\upsilon,1]}\circ \attackmodel\circ\hat{Y}=1|S=1}) + P({1_{[0,\upsilon}]\circ \attackmodel\circ\hat{Y}=0|S=0}))\\
        =&\frac{1}{2}(P({\hat{Y}\in \attackmodel^{-1}([\upsilon,1])|S=1}) + P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})\\
        =&\frac{1}{2}(1-P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})+P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})
        \label{eq:expbaeo}
    \end{align}
    }
    Then we use the total probability law for $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})$ and $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})$
    {
    \footnotesize
    \begin{align*}
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})\\
        =&P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=1})P(Y=1|S=1)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=0})P(Y=0|S=1)
    \end{align*}
    }
    {
    \footnotesize
    \begin{align*}
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})\\
        =&P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})P(Y=1|S=0)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})P(Y=0|S=0)\\
    \end{align*}
    }
     Because $\hat{Y}$ satisfies \eo we have 
    \begin{align*}
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=1})P(Y=1|S=1)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=0})P(Y=0|S=1)\\
        =&P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})P(Y=1|S=1)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})P(Y=0|S=1)\\
    \end{align*}
    
    Finally we substitute $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})$ and \\$P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})$ in equation 
    \ref{eq:expbaeo}.
    {
    \footnotesize
    \begin{align*}
        &\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))=\\
        &\frac{1}{2}
        P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})(P(Y=0|S=0) - P(Y=0|S=1))+\\
        &\frac{1}{2}P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})(P(Y=1|S=0) - P(Y=1|S=1))+\\
        &\frac{1}{2} = \\
        &\frac{1}{2}
        P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})(P(Y=0|S=0) - P(Y=0|S=1))+\\
        &\frac{1}{2}P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})(-P(Y=0|S=0) + P(Y=0|S=1))+\\
        &\frac{1}{2} = \\
        &\frac{1}{2}(P(Y=0|S=0) - P(Y=0|S=1))\\
        &\left(P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0}) - P(\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1)\right) +\\
        &\frac{1}{2}
    \end{align*}
    }
In conclusion, the balanced accuracy of $\hat{S}$ is equal to $\frac{1}{2}$ if and only if $P(Y=0|S=0) = P(Y=0|S=1)$ or $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0}) = P(\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1)$. So either $S$ is independent of $Y$ or $\hat{Y}$ is independent of $Y$.
\end{proof}


Hence, \eo is an effective defence mechanism only in the case where $S$ is independent of $Y$ or if is $\targetmodel$ has not learnt from $\traindata$ (classifier with random guess classification).
We note that in practice, these constraints are not met on real-world datasets. We present the independence of $Y$ and $S$ in by computing $|P(Y=0|S=0) - P(Y=0|S=1)|$ in Table~\ref{tab:indepYS}. A higher value indicates that $Y$ and $S$ are dependent. We note that in several cases, $S$ is dependent on $Y$.

\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{Independence of $Y$ and $S$ by reporting $|P(Y=0|S=0) - P(Y=0|S=1)|$: Higher value indicates that $Y$ and $S$ are dependent.
     }
    \begin{tabular}{|c|c|c|}
        \hline
        \rowcolor{LightCyan} \textbf{Dataset} & \textbf{\sex} &\textbf{\race}\\
        \hline
        \textbf{\compas}& 0.05 & 0.27\\
        \textbf{\census} & 0.20 & 0.13\\
        \textbf{\meps} & 0.07 & 0.13\\
        \textbf{\law} & 0.01 & 0.19\\
        \textbf{\credit} & 0.03 & 0.02\\
        \hline
    \end{tabular}
    \label{tab:indepYS}
\end{table}

Guided by Theorem~\ref{th:dpgood} and Theorem~\ref{th:eoo}, we conclude that only \demparity provides guarantees against \aia and can be used as an effective defence.
We will now validate these theoretical results empirically. 
%Guided by Theorem~\ref{th:dpgood} and the result on \eo, we conclude that \demparity is an effective defence against AIA.



==> New/misc/6.1evalattack.tex <==
\section{Evaluation: \adaptiveAIASoft and \adaptiveAIAHard}
\label{sec:evalAIA}


We evaluate the effectiveness of \adaptiveAIASoft and \adaptiveAIAHard in presence of class imbalance for $S(\omega)$ and show the advantage of using an adaptive threshold for soft labels and hard label over the state-of-the-art.


\noindent\textbf{\underline{\adaptiveAIASoft}} When $\targetmodel$ outputs soft labels, we consider the Song et al.~\cite{Song2020Overlearning} and Mahajan et al.~\cite{Mahajan2020DoesLS} as the state-of-the-art baselines to compare against. They use the default $\upsilon=0.5$ over $\attackmodel(\targetmodel(X(\omega)))$ where $\targetmodel(X(\omega))$ are soft labels.


\setlength\tabcolsep{1.5pt}
\begin{table}[!htb]
\caption{Comparing average balanced \aia accuracy over 25 runs for baseline with $\upsilon=0.5$~\cite{Song2020Overlearning,Mahajan2020DoesLS} and \adaptiveAIASoft.}
\label{tab:global_threshold_withoutsattr}
\begin{center}
\footnotesize
\begin{tabular}{ | c | c | c | c | c |  }
\hline
\rowcolor{LightCyan} 
\textbf{Dataset} & \textbf{Baseline ($\upsilon$=0.50)} & \textbf{\adaptiveAIASoft} \\ 
 \rowcolor{LightCyan} & \textbf{\race} | \textbf{\sex} & \textbf{\race} | \textbf{\sex} \\
\hline
\textbf{\census}& 0.50  | 0.53 &\textbf{ 0.58}| \textbf{0.64}\\
\textbf{\compas}& \textbf{0.59} | 0.50 &\textbf{0.59} | \textbf{0.64}\\
\textbf{\meps} & 0.56 | \textbf{0.56} &\textbf{0.59} |\textbf{0.56}\\
\textbf{\law}& 0.61 | \textbf{0.52} &\textbf{0.69} | \textbf{0.52}\\
\textbf{\credit}&0.50 | \textbf{0.55} &\textbf{0.51} | 0.53\\
\hline
\end{tabular}
\end{center}
\end{table}

We present the results in Table~\ref{tab:global_threshold_withoutsattr} for \race and \sex across all the datasets. We see that for the majority of the datasets, \adaptiveAIASoft is atleast as good as or better than the baseline. Hence, \adaptiveAIASoft is an effective \aia compared to prior work.

\noindent\textbf{\underline{\adaptiveAIAHard}} For hard labels, we consider the baseline of training a random forest model as $\attackmodel$ over hard labels to infer the value of $S(\omega)$ for a given $X(\omega)$. We present the effectiveness of \adaptiveAIAHard, fixed threshold over the hard labels, $\targetmodel(X(\omega))$.
We present the comparison of the baseline attack with \adaptiveAIAHard in Table~\ref{tab:global_threshold_withoutsattr_hard}.


\setlength\tabcolsep{1.5pt}
\begin{table}[!htb]
\caption{Comparison of baseline \aia (random forest trained to infer $S(\omega)$ using hard labels from $\targetmodel$ with \adaptiveAIAHard.}
\label{tab:global_threshold_withoutsattr_hard}
\begin{center}
\footnotesize
\begin{tabular}{ | c | c | c | c | c |  }
\hline
\rowcolor{LightCyan}
\textbf{Dataset} & \textbf{Baseline} & \textbf{\adaptiveAIAHard} \\ 
 \rowcolor{LightCyan} & \textbf{\race} | \textbf{\sex} & \textbf{\race} | \textbf{\sex} \\
\hline
\textbf{\census}& 0.50 | 0.50 & \textbf{0.56} | \textbf{0.59} \\ 
\textbf{\compas}& \textbf{0.61} | 0.50 & \textbf{0.61} | \textbf{0.57} \\ 
\textbf{\meps}& \textbf{0.55} | 0.50 & \textbf{0.55} | \textbf{0.52} \\ 
\textbf{\law}& 0.54 | \textbf{0.50} & \textbf{0.54} | \textbf{0.50} \\ 
\textbf{\credit}& 0.50 | \textbf{0.55} & \textbf{0.50} | \textbf{0.55} \\ 
\hline
\end{tabular}
\end{center}
\end{table}

We observe that in all cases, \adaptiveAIAHard is atleast as good as the baseline and in most cases outperforms the baseline. Hence, \adaptiveAIAHard is an effective attack to evaluate against.

==> New/misc/9conclusions.tex <==
\section{Discussion}\label{sec:conclusions}
 
\noindent\textbf{\underline{Summary of Contributions.}} We demonstrate the alignment of algorithmic group fairness and attribute privacy, crucial components for building trust in machine learning (ML). This reveals that training a model with algorithmic fairness can simultaneously offer attribute privacy against a blackbox \adv. We examine two scenarios where \adv obtains either soft or hard labels from $\targetmodel$, and we introduce improved \aia{s}: \adaptiveAIASoft and \adaptiveAIAHard.

Regarding \adaptiveAIASoft, we establish that \advdebias serves as a potent defense mechanism. It achieves fairness by ensuring indistinguishable predictions while accounting for a potential \adv during training. For \adaptiveAIAHard, we propose \egd with established fairness constraints: \demparity and \eo. Our theoretical and empirical analysis substantiates that \egddp is the optimal defense strategy against any \aia.

% addressing trade-offs between privacy, accuracy, fairness for soft labels

% \noindent\textbf{\underline{Limitations and Future Work.}} We enhance existing \aia{s} and introduce two attacks for $\targetmodel$'s outputs: soft labels (\adaptiveAIASoft) and hard labels (\adaptiveAIAHard). Our advancements surpass previous \aia{s}, although their optimality remains uncertain under the assumption of a powerful \adv with any possible background knowledge. As part of our future research, we are investigating the development of an optimal attack in this context. Moreover, creating a defense against an optimal \aia could assist in evaluating the optimality of current defenses and guide the formulation of more principled defenses.


==> New/misc/new/1introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Machine learning (ML) has been adopted in applications requiring high-stakes decision making, such as criminal justice, finance, and healthcare. The use of ML for such applications has raised concerns about their trustworthiness. Specifically, there are concerns about compromising user privacy~\cite{de2020overview} and the unfair decision-making~\cite{surveyfair}. Hence, it is crucial to design ML models satisfying both \textit{privacy and fairness} and explore whether their interaction is conflicting (i.e., trade-off) or aligned (i.e., reconciliation).

One privacy risk is where an adversary can infer sensitive attributes, e.g., \race and \sex, from ML model %observables (e.g., 
through predictions, parameters or intermediate outputs after deployment~\cite{fredrikson2,Mahajan2020DoesLS,yeom,Song2020Overlearning,malekzadeh2021honestbutcurious,MehnazAttInf}.  %during inference 
Such attacks, referred to as \textit{attribute inference attacks} (\aia{s}), pose a practical threat to data privacy and confidentiality. Let's consider a home loan company that aims to train an ML model to predict a customer's eligibility for a loan. The model uses various attributes, such as education, number of dependents, income, loan amount, and credit history, to make these predictions. To prevent bias in the allocation of home loans and potential redlining, the customer wishes to keep their \race private. However, if an attack can infer the \race of the customer, even though it is not directly part of the model training, it would violate the data privacy and confidentiality of the customer and creates the possibility of discrimination.

We classify \aia{s} in prior literature into: (i) imputation-based attacks, which exploit access to non-sensitive attributes, predictions, and background information~\cite{yeom,fredrikson2,MehnazAttInf,jayaraman2022attribute}, and (ii) representation-based attacks, which leverage distinguishability in predictions or intermediate outputs for different values of sensitive attributes~\cite{Song2020Overlearning,Mahajan2020DoesLS,malekzadeh2021honestbutcurious}. Jayaraman and Evans~\cite{jayaraman2022attribute} demonstrate that existing imputation-based attacks~\cite{yeom,fredrikson2,MehnazAttInf} are not more effective than data imputation and thereby do not pose a privacy risk. 

We study representation-based \aia{s} in a \textit{blackbox} scenario. Here, the adversary (\adv) submits inputs and can solely see the resulting target model's output predictions. \adv is unaware of the model's internal structure and parameters. We investigate two prediction types: (a) soft labels, presenting class probabilities, and (b) hard labels, deduced by selecting the class with the highest probability from soft labels. Here, the attack exploits the distinguishability with respect to different values of sensitive attribute from model's predictions for a given input data record. For instance, model predictions for \sex=male and \sex=female are different (see Figure~\ref{fig:distribution}). It is important to note that this distinguishability is often magnified by class imbalance in sensitive attributes within datasets, particularly in real-world applications~\cite{classIMb1,classIMb2}, an aspect that none of the prior \aia{s} take into account. Despite its widespread applicability, there has been a noticeable absence of prior works proposing effective defenses against \aia{s}.

On the other hand, algorithmic group fairness ensures that the model predictions are independent of the subgroups identified by some sensitive attributes (e.g., \race or \sex)~\cite{surveyfair}. This translates to ensuring that the predictions are indistinguishable for different values of sensitive attributes (e.g., males vs. females; whites vs. non-whites). For instance, adversarial debiasing (\advdebias)~\cite{debiase,NIPS2017_48ab2f9b} achieves fairness with respect to p\%-rule~\cite{fairmetric} while ensuring indistinguishablity in soft labels. Exponentiated gradient descent (\egd) with explicit fairness constraints for demographic parity (\demparity) or equalized odds (\eo) can achieve prediction indististinguishability for hard labels~\cite{reductions}.


We note that the objectives of algorithmic group fairness and attribute privacy are aligned: attribute privacy aims to minimize distinguishability in model predictions for various values of sensitive attributes, while group fairness seeks to ensure that model predictions remain independent of the sensitive attribute. Consequently, training a model with a group fairness constraint could potentially serve as a defense against \aia{s}.
In this work, we validate this conjecture and explore the design of an effective defence using fairness constraints against \aia{s}.



\noindent\textbf{\underline{Contributions.}} We study the interaction between attribute privacy and group fairness and claim the following contributions.
\begin{enumerate}[leftmargin=*]
    \item We quantify the risk of sensitive attribute leakage by proposing a blackbox \aia, \adaptiveAIA, which exploits the model's outputs while accounting for class imbalance in the sensitive attribute to improve attack success (Section~\ref{sec:adaptiveAIA}). We show the effectiveness of two variants of the attack depending on the model output: (a) \adaptiveAIASoft for soft labels, and (b) \adaptiveAIAHard for hard labels (Section~\ref{sec:evalAIA}). 
    \item As a defence against \adaptiveAIASoft, we present \advdebias (Section~\ref{sec:approachdef}) and empirically show that it lowers the distinguishability rendering the attack ineffective (Section~\ref{sec:evalDebias}). 
    \item As a defence against \adaptiveAIAHard, we present \egd with two well established fairness constraints: \demparity and \eo, as a defence against \aia{s}. We provide theoretical guarantees and limits of using \egd and identify \egddp as an effective defence (Section~\ref{sec:approachdef}). We empirically validate our theoretical guarantees (Section~\ref{sec:evalEGD}). We
    \begin{itemize}
        \item show that \adaptiveAIAHard does not degrade model utility, not increase the risk of membership inference attacks as suggested by Chang and Shokri~\cite{chang2021privacy} for \egdeo, and has a computational cost which will be naturally borne while satisfying regulatory requirements for fairness.
        \item conduct an extensive evaluation on how different factors impact the effectiveness of \egddp to show that \egddp is not impacted by \adv's background knowledge, the target model's architecture, and performs better than hard labels without fairness constraints.
    \end{itemize}
\end{enumerate}
We will open source our code upon publication.



==> New/misc/new/2background.tex <==

\section{Background}
\label{sec:background}

We present a background on ML and notations used in the rest of the paper (Section~\ref{back-ml}), followed by a discussion on \aia{s} (Section~\ref{sec:back-attribute}), and algorithmic fairness (Section~\ref{sec:back-fairness}).

\subsection{Machine Learning Classifiers}
\label{back-ml}

ML classification models, denoted as $\targetmodel^{\theta}$ ($\theta$ is omitted in the rest of the paper for simplicity), can be understood as functions parameterized by $\theta$ that map inputs with corresponding classification labels. $\theta$ is fine-tuned using a training dataset denoted as $\traindata$ with the objective is to minimize the loss incurred when predicting the classification label based on ground truth information.

Both $\traindata$ and the input data given to $\targetmodel$ consist of tuples. Each tuple contains non-sensitive attributes, sensitive attributes, and the actual classification label. Notably, we have removed sensitive attributes such as \race or \sex from both $\traindata$ and input data records to maintain privacy (i.e., censoring). Consequently, $\targetmodel$ is exclusively trained using non-sensitive attributes and the known correct classification labels. Sensitive attributes, although available for different data records, play no role in $\targetmodel$'s training or input data. They are reserved solely for the purpose of potential attacks (discussed later).

Once training is completed, input data records containing the non-sensitive attributes are passed to $\targetmodel$ to obtain the corresponding output in the form of a prediction scores (i.e., soft labels) denoted as $\targetmodel(X(\omega))$\footnote{We use this for both soft and hard labels.}.
The inputs passed during evaluation were not used during training and constitute the test dataset $\testdata$. It is used to evaluate how well $\targetmodel$ performs (i.e., accuracy) and generalizes.


Formally, consider a probability space $(\Omega, \mathcal{T}, \mathcal{P})$, measurable spaces $(E, \mathcal{U})$, $(\{0,1\},\mathcal{P}(\{0,1\}))$ and $([0,1], \mathcal{B})$ where $\mathcal{B}$ is the Borel tribe on $[0,1]$. We define random variables $X$ for the input data, $Y$ for the classification labels and $S$ for the sensitive attributes:
\begin{itemize}
    \item $X:(\Omega, \mathcal{T}, P) \longrightarrow (E, \mathcal{U}),$
    \item $Y:(\Omega, \mathcal{T}, P) \longrightarrow (\{0,1\},\mathcal{P}(\{0,1\})),$
    \item $S:(\Omega, \mathcal{T}, P) \longrightarrow (\{0,1\},\mathcal{P}(\{0,1\})),$
\end{itemize}
Consider the measurable function $\targetmodel:(E, \mathcal{U}) \longrightarrow ([0,1], \mathcal{B})$. 
It is used to build the statistic approaching $Y$. 
The parameters of $\targetmodel$ are updated by solving the optimization problem. 
The prediction of $\targetmodel$ is a random variable: $\hat{Y} = 1_{[\tau,1]}\circ \targetmodel\circ X$ where $\tau\in [0,1]$. 
%We consider a specific instance of random variables ($X(\omega), Y(\omega)$, $S(\omega)$) where $\omega$ is a parameter to generate different instances. 
We present a background on probability and measured spaces in Appendix~\ref{app:notations}.


\subsection{Attribute Inference Attacks}
\label{sec:back-attribute}

%Attacks which violate privacy and confidentiality in ML infer potentially sensitive unobservable information from observable information (e.g., model predictions). 
Attacks which violate privacy and confidentiality in ML infer potentially sensitive information from observable information (e.g., model predictions). 
This leakage of information is a privacy risk if \adv learns something about $\traindata$ -or the inputs- which would be impossible to learn without access to $\targetmodel$. This differentiates between a privacy risk and simple statistical inference~\cite{cormode}. 
Among the various privacy risks explored in literature pertaining to ML models, attribute inference attacks~\cite{fredrikson2,Mahajan2020DoesLS,yeom,Song2020Overlearning,malekzadeh2021honestbutcurious,MehnazAttInf} infer the specific value of a sensitive attribute for a specific input to ML model given some model observables (e.g., model predictions, parameters, intermediate layerwise outputs) and background information. Based on attack surface being exploited, \aia{s} can be categorized into (a) imputation-based attacks and (b) representation-based attacks. 

\noindent\textbf{\underline{Imputation-based attacks}} assume \adv has access to non-sensitive attributes in addition to model's predictions and background information (e.g., marginal prior over sensitive attribute and confusion matrix). We review these different imputation-based attacks below:



\setlength\tabcolsep{3pt}
\begin{table*}[!htb]
\caption{Comparison of prior work based on: attack surface exploited (e.g., model predictions ($\targetmodel(X(\omega))$), $X(\omega)$, $Y(\omega)$, distribution over $S(\omega)$ ($P_S$) and confusion matrix between true and predicted output across all training data records ($C(Y(\omega),\targetmodel(X(\omega)))$), whether $S(\omega)$ is censored, i.e., included in $\traindata$ or inputs, whether they account for class imbalance in $S(\omega)$, whether \adv is active or passive and whether the threat model is blackbox or whitebox. All the attacks assume the knowledge of auxiliary data $\auxdata$.}
\begin{center}
\footnotesize
\begin{tabular}{ |c|c|c|c|c|c| }
 \hline
 \rowcolor{LightCyan} 
 \textbf{Literature} & \textbf{Attack Vector} & \textbf{$S$ is censored?} & \textbf{Imbalance in $S$?} & \textbf{\adv} & \textbf{Threat Model} \\
 \hline
 \rowcolor{LightCyan} 
 \multicolumn{6}{|c|}{\textbf{Imputation-based Attacks}}\\
 \hline
 \textbf{Fredrikson et al.}~\cite{fredrikson2} & $X(\omega)$, $Y(\omega)$, $\targetmodel(X(\omega))$, \textbf{$P_S$}, $C(Y(\omega),\targetmodel(X(\omega)))$ & $\checkmark$ & $\times$ &  Passive & Blackbox\\
 \textbf{Yeom et al.}~\cite{yeom} & $X(\omega)$, $Y(\omega)$, $\targetmodel()$, \textbf{$P_S$} & $\checkmark$  & $\times$ &  Passive & Blackbox\\
  \textbf{Mehnaz et al.}~\cite{MehnazAttInf} & $X(\omega)$, $Y(\omega)$, $\targetmodel()$, \textbf{$P_S$}, $C(Y(\omega),\targetmodel(X(\omega)))$ & $\checkmark$ & $\times$ &  Passive & Blackbox\\
  \textbf{Jayaraman and Evans}~\cite{jayaraman2022attribute} & $X(\omega)$, $Y(\omega)$, $\targetmodel()$, \textbf{$P_S$}, $C(Y(\omega),\targetmodel(X(\omega)))$ & $\times$, $\checkmark$ & $\times$ &  Passive & Whitebox\\
  \hline
  \rowcolor{LightCyan} 
   \multicolumn{6}{|c|}{\textbf{Representation-based Attacks}}\\
  \hline
 \textbf{Song et al.}~\cite{Song2020Overlearning} & $\targetmodel(X(\omega))$ & $\times$ & $\times$ &  Passive & Both\\
 \textbf{Mahajan et al.}~\cite{Mahajan2020DoesLS} & $\targetmodel(X(\omega))$ & $\checkmark$ & $\times$ &  Passive & Blackbox\\
 \textbf{Malekzadeh et al.}~\cite{malekzadeh2021honestbutcurious} & $\targetmodel(X(\omega))$ & $\times$ & $\times$ &  Active & Blackbox\\
 \textbf{Our Work} & $\targetmodel(X(\omega))$ & $\times$, $\checkmark$ & $\checkmark$ &  Passive & Blackbox \\
 \hline
\end{tabular}
\end{center}
\label{tab:summary}
\end{table*}



\begin{itemize}[leftmargin=*]
    \item \textbf{Fredrikson et al.~\cite{fredrikson2}} assumes that \adv has access to $\targetmodel(X(\omega))$. 
    For this attack it is required that $X$ can be written $X = (\cdots,S,\cdots)$.
    We will refer to this case as "\textit{S is in the input}".
    Fredrikson et al. attack generates an input with different possible values of $S(\omega)$.
    It then chooses the most likely value based on $\targetmodel(X(\omega))$.

    \item \noindent\textbf{Yeom et al.~\cite{yeom}} assumes a distribution $P_S$ over $S$ which is used to estimate the value of $S$ for an arbitrary data record. They propose three different variants of \aia{s} based on assumptions on $P_S$: Attack 1 leverages membership oracle to determine the value of $S(\omega)$ and Attack 2 and 3 assume different types of distributions over $S$.
    For this attack to work, $S$ is in the input.
    
    \item \textbf{Mehnaz et al.~\cite{MehnazAttInf}} improves upon Fredrikson et al.~\cite{fredrikson1,fredrikson2} by exploiting $\targetmodel\circ X$ and $X$, with $S$ in the input. The attack relies on the intuition that $\targetmodel$'s output confidence is higher when the input has the correct value of $S$ as $\targetmodel$ encountered the target record with that attribute during training. Their attack involves generating multiple instances of input with different values of $S(\omega)$ (similar to Fredrikson et al.~\cite{fredrikson1,fredrikson2}) and identifying the most likely value of $S$. 
\end{itemize}

An appropriate baseline to identify whether such attacks are indeed a privacy risk is to use data imputation, i.e., train an ML model to infer value of missing attribute from other non-sensitive attributes without $\targetmodel(X(\omega))$~\cite{jayaraman2022attribute}. Jayaraman and Evans~\cite{jayaraman2022attribute} find that existing blackbox imputation-based attacks~\cite{yeom,fredrikson2,MehnazAttInf} do not perform any better than data imputation. In other words, the perceived privacy risk is actually stemming from statistical inference and hence not an actual privacy risk.

To address this, Jayaraman and Evans~\cite{jayaraman2022attribute} propose a whitebox \aia which outperforms prior blackbox attacks as well as data imputation in the setting where there is limited knowledge of data for \adv. However, since the attack is in a whitebox setting, we omit a detailed description of the attack. All these attacks require that: 

\begin{itemize}[leftmargin=*]
    \item $S$ is included in the input data records and $\traindata$ which is not always the case in realistic settings,
    \item $X(\omega)$ being attacked belong to $\traindata$.
\end{itemize}



\noindent\textbf{\underline{Representation-based attacks}} exploit the distinguishable intermediate layer outputs or predictions for different values of sensitive attributes~\cite{Song2020Overlearning,Mahajan2020DoesLS,malekzadeh2021honestbutcurious}. For instance, the distribution of $\targetmodel(X(\omega))$ for \textit{males} is different from the output prediction distribution for \textit{females}. We describe the existing attacks of this category below:

\begin{itemize}[leftmargin=*]
\item \textbf{Song et al.~\cite{Song2020Overlearning} / Mahajan et al.~\cite{Mahajan2020DoesLS}} assume that $S$ is not in the input. \adv only observes $\targetmodel\circ X$. \adv trains an ML attack model $\attackmodel$ to map the output predictions $\targetmodel(X(\omega))$ to $S(\omega)$.
In other words, the statistic $\hat{S}$ used to infer $S$ is of the form: $ \hat{S} = 1_{[0.5,1]}\circ \attackmodel\circ \targetmodel\circ X$, where $\attackmodel: [0,1]\rightarrow[0,1]$.


\item \textbf{Malekzadeh et al.~\cite{malekzadeh2021honestbutcurious}} considers the setting where \adv trains $\targetmodel$ with a special loss function to explicitly encode information about $S(\omega)$ in $\targetmodel(X(\omega))$.
It makes it easier to extract $S(\omega)$ during inference. In this setting, the model builder is malicious and actively introduces a ``backdoor''.
\end{itemize}

Our work focuses on representation-based \aia in a blackbox setting. We focus on Song et al.~\cite{Song2020Overlearning} and Mahajan et al.~\cite{Mahajan2020DoesLS} as our baselines. 
These attacks do not account for class imbalance in sensitive attribute commonly present in data from real-world applications which could effect \adv's attack success~\cite{classIMb1,classIMb2}.
In our evaluation, we consider an \aia using an adaptive threshold which outperforms these baselines attacks (Section~\ref{sec:evalAIA}).
Malekzadeh et al.~\cite{malekzadeh2021honestbutcurious} has a different threat model where \adv explicitly modifies the training to enhance the leakage of $S$. 
We do not assume such access to $\targetmodel$ in a blackbox setting. 
In addition, these attacks did not take into consideration the possibility to infer $S$ solely from the hard labels.
We summarize relevant prior work in Table~\ref{tab:summary}.



\subsection{Algorithmic Fairness}
\label{sec:back-fairness}

Algorithmic fairness aims at reducing biases in ML model predictions.
Indeed, data records belonging to certain subgroups influence $\targetmodel$'s predictions more than others.
For instance in criminal justice, the ethnicity of a culprit plays a non-negligible role in the prediction of them reoffending~\cite{fairjustice}. Generally, data records in the minority subgroup face unfair prediction behaviour compared to data records in the majority subgroup. These subgroups are identified based on a sensitive attribute (e.g., \race or \sex).
Those biases are learnt by $\targetmodel$ as they are part of the distribution of $\traindata$. 
There is two main categories of fairness of a ML model: 

% \begin{itemize}[leftmargin=*]
% \item \textbf{Individual fairness} ensures that two data records with same attributes except for $S$ have the same model prediction.
\textbf{Group fairness} adds constraints during training such that different subgroups (i.e., $S:\Omega\rightarrow\{0,1\}$) are treated equally. We focus our study on group fairness where $S$ represents either \sex or \race (i.e., $S(\omega)$ equals to 0 for woman, 1 for man, and 0 for black, 1 for white, respectively). There are different definitions of group fairness which have been introduced in prior work. We discuss two well-established and commonly used metrics: \demparity and \eo. 

%We focus our study on group fairness: let's explicit the two definitions of group fairness that we are going to use:

\begin{definition}
\label{def:dp}
    $\hat{Y}$ satisfies \demparity for $S$ if and only if: $P(\hat{Y}=0 | S=0) = P(\hat{Y}=0 | S=1)$.
    From that, we will call $|P(\hat{Y}=0 | S=0) - P(\hat{Y}=0 | S=1)|$ the dp-level of $\hat{Y}$.
\end{definition}


%\demparity is the historical definition of fairness but a perfect classifier (with perfect accuracy) does not respect the constraint if $Y$ is not independent of $S$~\cite{dpbad}.
%Hence, a perfect classifier is not considered fair according to \demparity~\cite{dpbad}.
%Hardt et al.~\cite{fairmetric2} proposed \eo as a modification of \demparity.

\demparity is the historical definition of fairness.
Legally, disparate impact is fairness definition recognized by law, where 80\% disparity is an agreed upon tolerance decided in the legal arena.
\demparity ensures that the number of correct prediction is the same for each population.
However, this may result in different false positive and true positive rates if the true outcome does actually vary with $S$~\cite{dpbad}.
Hardt et al.~\cite{fairmetric2} proposed \eo as a modification of \demparity to ensure that both the true positive rate and false positive rate will be the same for each population.

\begin{definition}
    \label{def:eo}
    $\hat{Y}$, classifier of $Y$, satisfies \eo for $S$ if and only if: $        \forall (\hat{y},y)\in\{0,1\}^2 \quad 
        P(\hat{Y}=\hat{y} | S=0,Y=y) = P(\hat{Y}=\hat{y} | S=1,Y=y)$.
\end{definition}

% If the classifier is binary, we generally use equality of opportunity.
% This definition only ensures that fairness is respected for the "priviledged outcome" \cite{fairmetric2}.

% \begin{definition}
%     \label{def:eop}
%     $\hat{Y}$, classifier of $Y$, satisfies \textbf{equality of opportunity} for the sensitive attribute $S$ if and only if:
%     \begin{equation}
%         \forall (\hat{y},y)\in\{0,1\}^2 \quad 
%         P(\hat{Y}=\hat{y}|S=0,Y=1) = P(\hat{Y}=\hat{y}|S=1,Y=1)
%     \end{equation}
% \end{definition}

% We remark that if $\hat{Y}$ satisfies \eo, then it satisfies equality of opportunity.
% This definition is used to make the under-constraint optimization problem easier to solve which is not a requirement in our case.
% Hence, we focus on disparate impact (Definition \ref{def:eo}) and \eo (Definition \ref{def:eo}).


The above fairness definitions can be achieved using three main fairness mechanisms: (a) pre-processing, (b) in-processing and (c) post-processing. \textit{Pre-processing} algorithms such as reweighing requires access to the training data and assigns weights to the data records to remove discrimination~\cite{preprocessing}.
\textit{In-processing} algorithms such as \advdebias~\cite{debiase} and \egd~\cite{reductions} add constraint during $\targetmodel$'s training to ensure fairness. %reductions
\textit{Post-processing} techniques, in turn, hide the bias in output predictions to satisfy the above fairness constraints but the underlying model is still biased. 

Similar to previous work~\cite{chang2021privacy}, we focus on in-processing algorithms.
%Unlike Chang et al.~\cite{chang2021privacy}, we however 
However, we consider not only EGD with \eo as fairness constraint but we also consider \demparity as fairness constraint and study the impact on privacy of \advdebias. 
% More specifically, we are going to show through a theoretical development and through an extensive empirical evaluation that the use of in-processing to impose \demparity is an effective defence against \aia{s}.


==> New/misc/new/3problem.tex <==
\section{Problem Statement}
\label{sec:problem}


We show why \aia{s} are effective in exploiting the distinguishability in $\targetmodel(X(\omega))$ for different values of $S(\omega)$ and motivate the need to account for class imbalance in $S(\omega)$ for a successful attack. We then describe the threat models we consider in this work.


%\noindent\textbf{\underline{Distinguishability in predictions.}} 
\subsection{Distinguishability in predictions}

Recall from Section~\ref{sec:back-attribute} that representation-based \aia{s} exploit the distinguishability in $\targetmodel(X(\omega))$ to infer $S(\omega)$ for an arbitrary input data record. To validate this, we plot the conditional densities of $\targetmodel\circ X$ for two subgroups, \race and \sex (each taking values $S=0$ and $S=1$), in Figure~\ref{fig:distribution} for multiple real-world datasets commonly used as benchmarks in fairness and privacy literature (detailed Section~\ref{sec:datasets}). 


\begin{figure}[!htb]
    \centering
    \begin{minipage}[b]{0.9\linewidth}
    \centering
    \subfigure[\census]{
    \includegraphics[width=1\linewidth]{figures/distributions/census_dist_withoutsattr.pdf}
    }
    \end{minipage}
    \begin{minipage}[b]{0.9\linewidth}
    \centering
    \subfigure[\compas]{
    \includegraphics[width=1\linewidth]{figures/distributions/compas_dist_withoutsattr.pdf}
    }
    \end{minipage}
    \begin{minipage}[b]{0.9\linewidth}
    \centering
    \subfigure[\law]{
    \includegraphics[width=1\linewidth]{figures/distributions/LAW_dist_withoutsattr.pdf}
    }
    \end{minipage}
    \begin{minipage}[b]{0.9\linewidth}
    \centering
    \subfigure[\meps]{
    \includegraphics[width=1\linewidth]{figures/distributions/meps_dist_withoutsattr.pdf}
    }
    \end{minipage}
    \begin{minipage}[b]{0.9\linewidth}
    \centering
    \subfigure[\credit]{
    \includegraphics[width=1\linewidth]{figures/distributions/credit_dist_withoutsattr.pdf}
    }
    \end{minipage}
    \caption{Distinguishable output predictions for two subgroups identified by \race and \sex. \adv exploits this to infer $S(\omega)$ for an arbitrary input data record.}
    \label{fig:distribution}
\end{figure}

Results show that $\targetmodel(X(\omega))$ are distinguishable for different values of $S(\omega)$, even when it is not included in the input. We observe that for \census, the distributions  over $\targetmodel(X(\omega))$ for both \race and \sex corresponding to the minority group (e.g., blacks and female) have a larger peak for lower output probability values.
This indicates that the classifier is likely to predict <50K salary for non-white and females compared to members of majority group.
For \compas, $\targetmodel$ is likely to predict males and blacks to re-offend compared to females or whites.
Furthermore, in \meps, the use of medical resources (visits to medical facility) is predicted as being lower for blacks and females.
$\targetmodel$'s discriminatory behaviour results in distinguishable output predictions for \adv which forms the basis of \aia{s} from $\targetmodel(X(\omega))$~\cite{Mahajan2020DoesLS,Song2020Overlearning}.


\noindent\textbf{Impact of Class Imbalance.} Class imbalance in $S(\omega)$ is commonly present in data from real-world applications~\cite{classIMb1,classIMb2}. To demonstrate this, we present the fraction of data records belonging to different subgroups categorized by \race or \sex in Table~\ref{tbl:bias}.
We observe that in some datasets the class imbalance is significant.

\setlength\tabcolsep{1.75pt}
\begin{table}[!htb]
 \footnotesize
\begin{center}
\caption{Summary of class imbalance in $S(\omega)$ across datasets.\label{tbl:bias}}
\begin{tabular}{ |c|c|c|c|c| }
\hline
\rowcolor{LightCyan} \textbf{Dataset} & \multicolumn{2}{c|}{\textbf{\sex}} & \multicolumn{2}{c|}{\textbf{\race}}\\
\rowcolor{LightCyan}  & \textbf{Male} & \textbf{Female} & \textbf{White} & \textbf{Non-White}\\
\hline
\textbf{\census} & 68\% & 32\% &90\%  & 10\%\\
\textbf{\compas} & 81\% & 19\% & 49\% & 51\%\\
\textbf{\law} & 57\% & 43\% & 94\% &6\% \\
\textbf{\meps} &53\%  & 47\% & 36\% & 64\% \\
\textbf{\credit} & 61\% & 39\% & 70\% & 30\%\\
 \hline
\end{tabular}
\end{center}
\end{table}

We conjecture that this bias is the main cause for the distinguishability in predictions for different subgroups which in turn affects the success of \aia{s}~\cite{classIMb1,classIMb2,classIMb3}. For instance, to correctly infer the value of $S(\omega)$, \adv can choose an appropriate threshold over $\attackmodel$'s predictions (ideally $0.5$ as seen in prior \aia{s}~\cite{Mahajan2020DoesLS,Song2020Overlearning}). However, this default threshold will yield poor attack success owing to the \textit{skew in $\targetmodel$ predictions.} Hence, the default threshold of 0.5 over $\attackmodel$'s predictions will not result in correct inference of $S(\omega)$. \adv's attack success can be improved by using an adaptive threshold~\cite{classIMb1,classIMb2,classIMb3}.
None of the prior attacks~\cite{Mahajan2020DoesLS,Song2020Overlearning} account for this. Hence, we consider the improved design of \aia{s} by using an adaptive threshold instead of using a default threshold (described Section~\ref{sec:adaptiveAIA}).

%\noindent\textbf{\underline{Threat Model.}} 

\subsection{Threat Model}

We present the assumptions about \adv's knowledge, training of $\targetmodel$ and attack methodology.

\noindent\textbf{\adv's Knowledge.} We consider a blackbox \adv with no knowledge of the target model's parameters or architecture.
%$\targetmodel$'s parameters or architecture. 
Moreover, we consider the case where the sensitive attribute is not used in the training procedure of the target model.
%$S(\omega)$ is censored, i.e., $S$ is not in the input. 
%$\targetmodel$ is trained on $\traindata$ which does not have $S(\omega)$ as a feature. 
%\adv 
The adversary has access to the output of the target model which can be either in the form of a soft label (i.e., a real number representing the prediction score) or a hard label (i.e., an expression of the predicted label).  
%The former we model by the random variable $\targetmodel\circ X$ and for the latter we add to the model an indicator function to obtain an expression of the prediction of the label: 
%$ \hat{Y}=1_{[\tau,1]}\circ \targetmodel\circ X$.
% AB: not possible to say it more easily?
%in the intro: (a) soft labels, presenting class probabilities, and (b) hard labels, deduced by selecting the class with the highest probability from soft labels.
\adv has access to $\auxdata$ sampled from the same distribution as $\traindata$. This is a common assumption in prior \aia{s}~\cite{Mahajan2020DoesLS,Song2020Overlearning,yeom}. 
We consider the case where $\auxdata$ might be sampled from a different distribution Section~\ref{sec:otherfactors}.
%$Q$ than the $\traindata$'s distribution $P$ which we discuss later. 
%We consider the case where $\auxdata$ might be sampled from a different distribution $Q$ than the $\traindata$'s distribution $P$ which we discuss later. 
$\auxdata$ is split into two disjoint datasets: $\auxtraindata$ used for designing the attack and $\auxtestdata$ to evaluate the attack success.



\noindent\textbf{Training $\targetmodel$.} We assume that $\targetmodel$ is trained with fairness constraints. We consider two ways to achieve fairness: (a) adversarial debiasing (\advdebias)~\cite{NIPS2017_48ab2f9b,debiase} and (b) exponentiated gradient descent (\egd)~\cite{reductions}.

\begin{itemize}[leftmargin=*]
    \item \textbf{\advdebias} empirically achieves fairness by training $\targetmodel$ to have indistinguishable output predictions. In addition to $\targetmodel$, a discriminator network $f_{disc}$ is train to infer $S(\omega)$ corresponding to an input $X(\omega)$ given $\targetmodel(X(\omega))$. $\targetmodel$ is then trained to minimize the success of $f_{disc}$, i.e., predictions are indistinguishable between different values of $S(\omega)$. Note that \advdebias outputs \textit{soft labels}.

    \item \textbf{\egd} solves an under-constraint optimization problem to find a collection of optimal measurable functions $t_0, \cdots, t_{N-1}$ and threshold $(\tau_0,\cdots\tau_{N-1})\in[0,1]^N$.
These are used to create the statistic $\hat{Y}$ that estimates ground truth labels $Y$.
To do so, a random variable $I:\Omega\rightarrow\{0,\cdots,N-1\}$ is used to select one of the measurable function. At the end of this process, \egd for fair classification outputs a randomized classifier of the form: $\hat{Y} = 1_{[\tau_I, 1]}\circ t_I\circ X$. $\targetmodel$ when trained using \egd outputs \textit{hard labels}, i.e., $argmax$ over $\targetmodel(X(\omega))$. To ensure fairness, \egd is trained to satisfy different fairness constraints (e.g., \demparity or \eo).
\end{itemize}




\input{fig_tm2}

\noindent\textbf{Attack Methodology} \adv trains $\attackmodel$ on $\auxtraindata$ (non-overlapping dataset with $\traindata$ available to \adv) to infer $S(\omega)$ using $\targetmodel(X(\omega))$. $\attackmodel$ is then evaluated on $\auxtestdata$. This is shown in Figure~\ref{fig:tm2}. This attack is applicable in both cases when $\targetmodel$'s outputs are soft and hard labels.

Given a collection of hard labels from $\targetmodel$, $\hat{Y}_h(\omega_0),\cdots,\hat{Y}_h(\omega_{A-1})$, available to \adv, \adv can then build a statistic $\hat{S}$ to infer $S$: $ \hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y}_h\circ X$. 
Similarly, for soft labels $\hat{Y}_s(\omega_0),\cdots,\hat{Y}_s(\omega_{A-1})$, \adv builds a statistic $\hat{S}$ to infer $S$: $ \hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y}_s\circ X$. 
Here, $\upsilon \in [0,1]$ is a threshold which is optimized to improve \adv's attack success.



% \item \label{threatmodel2} 
% \adv has access to a collection of 
% $A$ data records \\ $\targetmodel(X(\omega_0)), \cdots, \targetmodel(X(\omega_{A-1}))$ she is attacking.\\
% $\targetmodel(X(\omega))$ is often referred as \textit{soft label} in the literature.
% \adv also has access to $\auxdata$: one realization of an independent identically distributed sample of the joint law $Q_{\targetmodel\circ X,S}$, where $Q$ is a probability measure on $(\Omega, \mathcal{T})$.
% Using $\auxdata$, she trains a ML model $a:[0,1]\rightarrow[0,1]$ to minimize a loss function on the auxilary dataset (e.g., mean square error). \adv can then build a statistic $\hat{S}$ to infer $S$:
% \begin{equation}
%     \label{eq:tm1}
%     \hat{S}=1_{[\upsilon,1]}\circ a\circ \targetmodel\circ X,
% \end{equation}
% where $\upsilon \in [0,1]$ is a threshold that can be learned to account for class imbalance.
% \end{enumerate}

%In both threat models, we assume that \adv has access to a non-overlapping auxiliary dataset. In both cases, the attack model is trained using $\auxdata$.
%It is then used to attack data records after inference has been made by $\targetmodel$ $\targetmodel$ trained on the target dataset. 



%\subsection{Why is this a Privacy Risk?}
%\label{sec:whyprivacy}

%\aia{s} have been established as a privacy threat by several prior works~\cite{Song2020Overlearning,jayaraman2022attribute,Mahajan2020DoesLS,malekzadeh2021honestbutcurious}.
%However, for imputation-based attacks, Jayaraman and Evans~\cite{jayaraman2022attribute} show that these attacks are no better than data imputation. Hence, the perceived privacy risk is mainly from statistical inference. However, statistical inference should be considered as a privacy risk if access to f target allows for a more accurate personal information inference about an individual, regardless of whether or not they were included in $\mathcal{D}_{train}$~\cite{cormode}.
%However, statistical inference should be considered as a privacy risk when \adv doesn'\targetmodel have access to the input data, even more if $S(\omega)$ isn'\targetmodel included in the input, as in both of our threat models.

%\aia{s} have been established as a privacy threat by several prior works [31], [20], [8], [26]. However, for imputation-based attacks, Jayaraman and Evans [20] show that these attacks are no better than data imputation. Hence, the perceived privacy risk is mainly from statistical inference and adversary’s access to f target is not exploited to the fullest. However, statistical inference should be considered as a privacy risk if access to f target allows for a more accurate personal information inference about an individual, regardless of whether or not they were included in $\mathcal{D}_{train}$ [6].



==> New/misc/new/4approach.tex <==
\section{\adaptiveAIA: \aia with Adaptive Threshold}
\label{sec:adaptiveAIA}

Having motivated the need to account for class imbalance, we first present \adaptiveAIA, an \aia with adaptive threshold. We consider two variants of the attack, \adaptiveAIASoft for soft labels, and \adaptiveAIAHard for hard labels. We describe these attacks below.

\noindent\textbf{\underline{\adaptiveAIASoft}} Recall that prior \aia{s}~\cite{Song2020Overlearning,Mahajan2020DoesLS} use the default classification threshold of $0.5$ over $\attackmodel\circ \targetmodel\circ X$. As discussed previously, given the skew in sensitive attribute, we conjecture that the default threshold is likely to not have the best \aia success.
To overcome this limitation, we present \adaptiveAIASoft, with \textit{adaptive threshold} over the soft labels to account for any differences due to imbalance in $S(\omega)$. \adv computes the optimal threshold $\upsilon^*$ on $\auxtraindata$ which is later used for attack.

We compute $\upsilon^*$ to balance true positive rate (TPR) and false positive rate (FPR). Formally, $TPR_{\upsilon} = P(\hat{S}=1 | S=1)$ and $FPR_{\upsilon} = P(\hat{S}=1 | S=0)$, where $\hat{S}$ is defined in function of $\upsilon$ (see threat model in Section~\ref{sec:problem}). Ideally, a perfect attack would result in no FPR (i.e., a rate of 0) and only TPR (i.e., a rate of 1).
\adv's goal is thus to approach this optimal value of TPR and FPR.
Formally, $\upsilon^*\in[0,1]$ where $\upsilon^* = \text{argmin}_{\upsilon} (1-TPR_\upsilon)^2 + FPR_\upsilon^2$.

We define the receiver operating characteristic ($\textsc{roc}$) curve as a function which maps each $\upsilon$ to the corresponding FPR and TPR values:
\begin{equation*}
    \textsc{roc}: \left\{
    \begin{matrix}
       [0,1]\longrightarrow \left[0,1\right]^2\\
       \upsilon\mapsto (FPR_\upsilon,TPR_\upsilon)
    \end{matrix}
    \right.
\end{equation*}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\linewidth]{image/roc.pdf}
    %\includegraphics[width=0.5\linewidth]{figures/curve_w_tau/CENSUS/roc.pdf}
    \caption{ROC curve for \law to infer \race: an adaptive threshold can lower the FPR.}
    \label{fig:curvesROC}
\end{figure}

For illustration purposes, we plot the ROC curve for inferring \race attribute on \law in Figure~\ref{fig:curvesROC}.
We indicate TPR and FPR for $\upsilon= 0.5$ and $\upsilon^*$. 
We observe that $\upsilon^*$ does not correspond to the default classification threshold of $0.5$ used in the literature.
We later show that calibrating the threshold improves the attack success (Section~\ref{sec:evalAIA}).


\noindent\textbf{\underline{\adaptiveAIAHard}} In the case of infering the sensitive attribute from hard labels, it is not necessary to train a machine learning model.
Indeed, the set of functions from $\{0,1\}$ to $\{0,1\}$ contains only four elements : 
 $x\mapsto 0$, $x\mapsto x$, $x\mapsto 1-x$, and $x\mapsto 1$.
 Hence we are assured to obtain the most efficient attack by trying out each of those functions and choosing the one which gives the best balanced accuracy.

%Instead of training $\attackmodel$ which maps $\{0,1\}$ to $\{0,1\}$, the hard labels for the binary classification allows to predict $S(\omega)$ directly. Those four functions mapping input to output are: $x\mapsto 0$, $x\mapsto x$, $x\mapsto 1-x$, and $x\mapsto 1$.
%Consequently, we can test each of them to find the function which gives the highest balanced \aia accuracy. Hence, here we do not require any additional threshold optimization. 


%\noindent\textbf{\underline{\adaptiveAIAHard}} Instead of training $\attackmodel$ which maps $\{0,1\}$ to $\{0,1\}$, the hard labels for the binary classification allows to predict $S(\omega)$ directly. Those four functions mapping input to output are:
%\begin{itemize}
%\item $b_0:x\mapsto 0$
%\item $b_1:x\mapsto x$
%\item $b_2:x\mapsto 1-x$
%\item $b_3:x\mapsto 1$
%\end{itemize}
%In contrast to soft labels, we can find an attack which gives the highest balanced \aia accuracy. Hence, here we do not require any additional threshold optimization. 
%We present \adaptiveAIAHard in Algorithm~\ref{algo:22}.
%\begin{algorithm}
%    \caption{Optimal attack in $B_{2\rightarrow 2}$}
%    \label{algo:22}
%    \begin{algorithmic}
%        \State $b\gets b_0$
%        \For{$i \gets 1,2,3$}
%            \If{$BA(b_i)>BA(b)$}
%                \State $b\gets b_i$
%            \EndIf
%        \EndFor
%        \State \Return $b$
%    \end{algorithmic}
%\end{algorithm}




















\section{Attribute Privacy via Fairness}\label{sec:approachdef}



We motivate the use of algorithmic fairness to mitigate \aia{s}. We then describe the theoretical results evaluating the effectiveness of \egd with \demparity and \eo as a defence against \adaptiveAIA. We also show in the Appendix~\ref{app:dp} that Differential Privacy (DP) in the context of machine learning gives no guarantee of protection against attribute privacy.


\noindent\textbf{\underline{Motivation}} Attribute privacy, i.e., resistance against \aia{s} requires $\targetmodel$'s predictions indistinguishable for different values of $S(\omega)$. Fairness algorithms such as \advdebias achieve this empirically where $\targetmodel$ is trained to output indistinguishable predictions (soft labels) for sensitive attributes. \egd, on the other hand, adds an additional constraint during training to ensure indistinguishable predictions (hard labels). Hence, we conjecture algorithmic fairness to act as a defence against \aia. In other words, training for fairness can help achieve attribute privacy due to their \textit{aligned} objectives.


\noindent\textbf{\underline{Mitigating \adaptiveAIASoft with \advdebias}} On training a model with \advdebias, we expect the model predictions (soft labels) to be indistinguishable compared to the case when model is trained without \advdebias (i.e., Figure~\ref{fig:distribution}). We present similar plots after training $\targetmodel$ with \advdebias in Figure~\ref{}. We find that in all the cases, the prediction distribution for different values of sensitive attributes are indistinguishable. Hence, we expect that an \adv with access to soft labels from $\targetmodel$ should not be able to infer $S(\omega)$. We empirically verify this in Section~\ref{}


\noindent\textbf{\underline{Mitigating \adaptiveAIAHard with \egd}} Recall that $\targetmodel$ can be trained with \egd to satisfy either \demparity or \eo. Different fairness definitions give different guarantees on mitigating \aia{s}. We theoretically evaluate the balanced \aia accuracy under both \demparity and \eo fairness constraints.


\begin{theorem}
\label{th:dpgood}
%If $\hat{Y}$ satisfies \demparity for $S$ then 
%for all attack model $\attackmodel:[0,1]\rightarrow[0,1]$ and for all threshold $\upsilon\in[0,1]$,
%the balanced \aia accuracy of~$\hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y}$ is equal to $\frac{1}{2}$
The maximum balanced \aia accuracy achievable is equal to $\frac{1}{2}(1+\text{dp-level of the $\targetmodel$})$ . 
\end{theorem}

\begin{proof}
We have seen in section \ref{sec:atthard} that the set $B$ of function from $\{0,1\}$ to $\{0,1\}$ contains four elements $b_0$, $b_1$, $b_2$ and $b,3$.
For every $b\in B$ the balanced \aia accuracy is 
$BA(b) = \frac{1}{2}(P(b\circ \hat{Y}=0|S=0) + P(b\circ \hat{Y}=1|S=1))$.
We have $BA(b_0) = BA(b_3) = \frac{1}{2}$ hence we can discard those elements when solving the attack optimisation problem.
This problem writes $\text{max}_{b\in B}B(A(b)) = \text{max}(BA(b_1), BA(b_2))$.
We remark that $b_1\circ \hat{Y}=\hat{Y}$ and $b_2\circ \hat{Y}=1 - \hat{Y}$.
Hence,
{\footnotesize
\begin{align*}
    BA(b_1) &= \frac{1}{2}(P(\hat{Y}=0|S=0) + P(\hat{Y}=1|S=1))\\
    &=\frac{1}{2}(1+P(\hat{Y}=1|S=1) - P(\hat{Y}=1|S=0))
\end{align*}
}
And
{\footnotesize
\begin{align*}
    BA(b_2)=\frac{1}{2}(1+P(\hat{Y}=1|S=0) - P(\hat{Y}=1|S=1))
\end{align*}
}
Thus,
{\footnotesize
\begin{align*}
    &\text{max}_{b\in B}BA(b) \\
    = &\frac{1}{2}\left(1+\text{max}\left(
    \begin{matrix}
        P(\hat{Y}=0|S=0) -P(\hat{Y}=1|S=1)\\ 
        P(\hat{Y}=1|S=0) -P(\hat{Y}=0|S=1)
    \end{matrix}
    \right)\right)\\
    =&\frac{1}{2}(1+|P(\hat{Y}=1|S=1) - P(\hat{Y}=1|S=0)|)
\end{align*}
}
%Let $\hat{Y}:\Omega\rightarrow\{0,1\}$ be a random variable that satisfies \demparity for $S$ and $\hat{S}$ be the inferred sensitive attribute from the attack classifier on exploiting $\hat{Y}$. Then,
%\begin{equation}
%\label{eq:defShat}
%    \hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y},
%\end{equation}
%where $\upsilon\in[0,1]$ and $\attackmodel:\{0,1\}\rightarrow[0,1]$ is a measurable function.

%We compute the balanced \aia accuracy to infer $\hat{S}$, given by, $\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))$.
%In this expression, we substitute the definition of $\hat{S}$ from Equation~\ref{eq:defShat} which gives us the conditional law of $Y$ knowing $S$.
%Using the Definition~\ref{def:dp}, we can compute the balanced \aia accuracy when training with \demparity.
%{
%\footnotesize
%\begin{align*}
%    &\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))\\
%    =&\frac{1}{2}(P({1_{[\upsilon,1]}\circ \attackmodel\circ\hat{Y}=1|S=1}) + %P({1_{[0,\upsilon]}\circ \attackmodel\circ\hat{Y}=0|S=0}))\\
%    =&\frac{1}{2}(P({\hat{Y}\in \attackmodel^{-1}([\upsilon,1])|S=1}) + P({\hat{Y}\in %\attackmodel^{-1}([0,\upsilon])|S=0})\\
%    =&\frac{1}{2}(1-P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})+P({\hat{Y}\in %\attackmodel^{-1}([0,\upsilon])|S=0})\\
%    =&\frac{1}{2}(1-P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})+P({\hat{Y}\in %\attackmodel^{-1}([0,\upsilon])|S=0})\\
%    =&\frac{1}{2}
%\end{align*}
%}
\end{proof}
In summary, satisfying \demparity indicates that the dp-level is zero, consequently, \textbf{if $\targetmodel$ satisfies \demparity then no $\attackmodel$ will perform better than a random guess}. Hence, \demparity can ensure the confidentiality of $S(\omega)$.
We now present the balanced \aia accuracy under \eo constraint.

\begin{theorem}
\label{th:eoo}
If $\hat{Y}$ satisfies \eo for $Y$ and $S$ then for all attack model $\attackmodel:[0,1]\rightarrow[0,1]$ and for all threshold $\upsilon\in[0,1]$, the balanced \aia accuracy of $\hat{S}=1_{[\upsilon,1]}\circ \attackmodel\circ \hat{Y}$ is greater than $\frac{1}{2}$. In addition, balanced \aia accuracy is random guess $\frac{1}{2}$ if and only if $Y$ is independent of $S$ or $\hat{Y}$ is independent of $Y$.
\end{theorem}

\begin{proof}
    Let $\hat{Y}:\Omega\rightarrow\{0,1\}$ a random variables classifier of $Y$ that satisfies \eo for $S$.
    Let $\hat{S}$ an attack classifier of $S$ using $\hat{Y}$ with the same definition as in equation \ref{eq:defShat}.
    For this proof, we use the total probability law to make use of the conditional law of $\hat{Y}$ knowing $(S,Y)$.
    {
    \footnotesize
    \begin{align}
         &\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))\\
        =&\frac{1}{2}(P({1_{[\upsilon,1]}\circ \attackmodel\circ\hat{Y}=1|S=1}) + P({1_{[0,\upsilon}]\circ \attackmodel\circ\hat{Y}=0|S=0}))\\
        =&\frac{1}{2}(P({\hat{Y}\in \attackmodel^{-1}([\upsilon,1])|S=1}) + P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})\\
        =&\frac{1}{2}(1-P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})+P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})
        \label{eq:expbaeo}
    \end{align}
    }
    Then we use the total probability law for $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})$ and $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})$
    {
    \footnotesize
    \begin{align*}
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})\\
        =&P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=1})P(Y=1|S=1)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=0})P(Y=0|S=1)
    \end{align*}
    }
    {
    \footnotesize
    \begin{align*}
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})\\
        =&P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})P(Y=1|S=0)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})P(Y=0|S=0)\\
    \end{align*}
    }
     Because $\hat{Y}$ satisfies \eo we have 
    \begin{align*}
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=1})P(Y=1|S=1)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1,Y=0})P(Y=0|S=1)\\
        =&P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})P(Y=1|S=1)+\\
        &P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})P(Y=0|S=1)\\
    \end{align*}
    
    Finally we substitute $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=1})$ and \\$P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0})$ in equation 
    \ref{eq:expbaeo}.
    {
    \footnotesize
    \begin{align*}
        &\frac{1}{2}(P(\hat{S}=1|S=1)+P(\hat{S}=0|S=0))=\\
        &\frac{1}{2}
        P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})(P(Y=0|S=0) - P(Y=0|S=1))+\\
        &\frac{1}{2}P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})(P(Y=1|S=0) - P(Y=1|S=1))+\\
        &\frac{1}{2} = \\
        &\frac{1}{2}
        P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0})(P(Y=0|S=0) - P(Y=0|S=1))+\\
        &\frac{1}{2}P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1})(-P(Y=0|S=0) + P(Y=0|S=1))+\\
        &\frac{1}{2} = \\
        &\frac{1}{2}(P(Y=0|S=0) - P(Y=0|S=1))\\
        &\left(P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0}) - P(\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1)\right) +\\
        &\frac{1}{2}
    \end{align*}
    }
In conclusion, the balanced accuracy of $\hat{S}$ is equal to $\frac{1}{2}$ if and only if $P(Y=0|S=0) = P(Y=0|S=1)$ or $P({\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=0}) = P(\hat{Y}\in \attackmodel^{-1}([0,\upsilon])|S=0,Y=1)$. So either $S$ is independent of $Y$ or $\hat{Y}$ is independent of $Y$.
\end{proof}


Hence, \eo is an effective defence mechanism only in the case where $S$ is independent of $Y$ or if is $\targetmodel$ has not learnt from $\traindata$ (classifier with random guess classification).
We note that in practice, these constraints are not met on real-world datasets. We present the independence of $Y$ and $S$ in by computing $|P(Y=0|S=0) - P(Y=0|S=1)|$ in Table~\ref{tab:indepYS}. A higher value indicates that $Y$ and $S$ are dependent. We note that in several cases, $S$ is dependent on $Y$.

\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{Independence of $Y$ and $S$ by reporting $|P(Y=0|S=0) - P(Y=0|S=1)|$: Higher value indicates that $Y$ and $S$ are dependent.
     }
    \begin{tabular}{|c|c|c|}
        \hline
        \rowcolor{LightCyan} \textbf{Dataset} & \textbf{\sex} &\textbf{\race}\\
        \hline
        \textbf{\compas}& 0.05 & 0.27\\
        \textbf{\census} & 0.20 & 0.13\\
        \textbf{\meps} & 0.07 & 0.13\\
        \textbf{\law} & 0.01 & 0.19\\
        \textbf{\credit} & 0.03 & 0.02\\
        \hline
    \end{tabular}
    \label{tab:indepYS}
\end{table}

Guided by Theorem~\ref{th:dpgood} and Theorem~\ref{th:eoo}, we conclude that only \demparity provides guarantees against \aia and can be used as an effective defence.
We will now validate these theoretical results empirically. 
%Guided by Theorem~\ref{th:dpgood} and the result on \eo, we conclude that \demparity is an effective defence against AIA.



==> New/misc/new/5setup.tex <==
\section{Experimental Setup}
\label{sec:setup}


\noindent\textbf{\underline{Datasets}}
\label{sec:datasets} We consider five real-world datasets covering different domains including criminal justice, income prediction, healthcare, college performance and credit applications, to illustrate the effectiveness of the proposed \aia{s}.
These datasets have been used as a benchmark in attribute privacy~\cite{Song2020Overlearning,MehnazAttInf,Mahajan2020DoesLS} and fairness literature~\cite{surveyfair}.

\noindent\textbf{US adult income dataset (\census)} comprises of 30,940 data records with 95 attributes about individuals from 1994 US Census data.
The attributes include marital status, education, occupation, job hours per week among others.
The classification task is to estimate whether an individual makes an income of 50k per annum. For $\targetmodel$, we use 24,752 data records for $\traindata$ and 6,188 data records as $\testdata$. We use 4,950 data records from $\testdata$ as $\auxtraindata$ for training $\attackmodel$ and evaluate it on 1,238 unseen data records in $\auxtestdata$.


\noindent\textbf{Recidivism dataset (\compas)} is used for commercial algorithms by judges and parole officers for estimating the likelihood of a criminal re-offending.
The classification task is binary: whether a criminal will re-offend or not, and contains 6,172 criminal defendants in Florida. The dataset contains 7 attributes and we use 4,937 data records for training $\targetmodel$ and 1,235 data records as testing dataset. We use 988 data records from $\testdata$ as $\auxtraindata$ for training $\attackmodel$, i.e., $\auxtraindata$ and evaluate it on 247 unseen data records in $\auxtestdata$.


\noindent\textbf{Medical Expenditure Panel Survey dataset (\meps)} contains 15,830 records of different patients using medical services by capturing the trips made to clinics and hospitals.
The classification task is to predict the utilization of medical resources as 'High' if the sum of the number of office based visits, outpatient visits, ER visits, inpatient nights and home health visits, is greater than 10. We use 12,664 data records for training $\targetmodel$ and 3,166 $\traindata$ records as testing dataset. We use 2,532 data records from $\testdata$ as $\auxtraindata$ for training $\attackmodel$ and evaluate it on 634 unseen data records in $\auxtestdata$.

\noindent\textbf{Law school dataset (\law)} contains information on 20,460 law students such as their entrance exam scores (LSAT), their grade-point average (GPA) collected prior to law school, and their first year average grade. The data is collected based on a survey conducted by Law School Admission Council across 163 law schools in the United States. 
Given this data, a school predicts if an applicant will have a high first year average grade. The dataset has four attributes and we use 16,368 data records as $\traindata$ for training $\targetmodel$ and 4,092 data records for $\testdata$. We use 3,273 data records from $\testdata$ as $\auxtraindata$ for training $\attackmodel$ and evaluate it on 819 unseen data records in $\auxtestdata$.

\noindent\textbf{UCI Credit Card dataset (\credit)} is from the UCI ML dataset repository and contains information about different credit card applicants. The classification task is binary indicating whether the application was approved or not. The dataset contains 30,000 records with 24 attributes for each record. We use 24,000 data records for training $\targetmodel$ and 6,000 as $\testdata$. We use 4,800 data records from $\testdata$ as $\auxtraindata$ for training $\attackmodel$ and evaluate it on 1,200 unseen data records in $\auxtestdata$.

%\begin{table}[!htb]
%\footnotesize
%\begin{center}
%\caption{Summary of dataset splits.}
%\begin{tabular}{ | c | c | c | c | c |}
%\hline
%\rowcolor{LightCyan}  \textbf{Dataset} & |$\traindata$| & |$\testdata$| & |$\auxtraindata$| & |$\auxtestdata$|\\ 
%\hline
% \textbf{\census} & 24,752 & 6,188 & 4,950 & 1,238\\  
% \textbf{\compas} & 4,937 & 1,235 &988 & 247\\  
%\textbf{\meps} & 12,664 & 3,166 & 2,532 & 634\\  
% \textbf{\law} & 16,368 & 4,092 & 3,273 & 819\\  
%\textbf{\credit} & 24,000 & 6,000 & 4,800 & 1,200\\  
%  \hline
%\end{tabular}
%\end{center}
%\label{tab:dataset}
%\end{table}

We summarize the dataset splits in Annex~\ref{app:dataset}. %Table~\ref{tab:dataset}. 
In all the datasets, we consider the \sex (``Male and Female'') and \race (``White and Non-White'') as the sensitive binary attributes. For \credit, we use the \textsc{Age} attribute classified as ``Young'' or ``Old'' as sensitive. For brevity, we refer to the \textsc{Age} attribute as \race in evaluation tables. \\

%model architectures and hyperparameters

\noindent\textbf{\underline{Methodology}}
\label{sec:methodology} We report the results corresponding to the average over ten repetitions with cross validation for each experiment. All the experiments have been parallelized and executed on a hybrid GPU/CPU computing farm. We implement our code using sklearn~\footnote{\url{https://scikit-learn.org/}}. For training the model with fairness constraints, we use fairlearn library~\footnote{\url{https://fairlearn.org/}}. 

\noindent\textbf{$\targetmodel$ Classification Accuracy.} We train the ML models (i.e., a scikit-learn implementation of random forest with default settings) on primary classification tasks for all the five datasets. We found the baseline balanced accuracy is 76.84\% for \census, 73.64\% for \compas,  67.87\% for \meps, and 52.74\% for \law and 70.86\% for \credit.

\noindent\textbf{$\targetmodel$ Architecture.} We focus on random forest as in prior work~\cite{chang2021privacy} with 100 trees. We also evaluate against a perceptron, a neural network with one layer. These models were sufficient to achieve state-of-the art performance. See discussion (Section~\ref{sec:discussions}) for evaluation on complex model trained on high-dimensional dataset.

\noindent\textbf{Statistical Significance}. We conducted a statistical test (i.e., ANOVA) to check for statistical significance of the results (i.e., p-value <0.05). In other words, for p-value<0.05 the difference is statistically significant else the results are indistinguishable. We present the p-values along with the results wherever necessary.\\



% \subsubsection{Membership Inference Attack}
% \label{sec:methodoMIA}

% To get a full picture of the impact of \egd on privacy, we also evaluate the influence of this fair classification strategy on the success of membership inference attacks. 
% A membership inference attack aims to identify whether a particular target data record was used to train the model. %~\cite{miasurvey}.
% Practically, this attack leverages the fact that ML model tends to produce results with more confidence on their $\mathcal{D}_{train}$, especially if the model is overfitted.
% Different methodologies have been proposed to conduct a membership inference attack, by looking at the difference in loss between training and non-training data records~\cite{yeom}, or by using one or multiple shadow models~\cite{meminf,carlini2022membership}.
% In our case, we consider a methodology similar to Yeom et al.~\cite{yeom} which used the difference of the model loss between the prediction $\targetmodel\circ X$ and ground truth label $Y$.


% We train an attack classifier to infer if a data record is a member of the training set of $\targetmodel$.
% This attack classifier is trained on dataset containing the error made by $\targetmodel$.
% Formally, we train the attack classifier $m:[-1,1]\rightarrow[0,1]$ to minimize a mean square error loss on 
% $m\circ (t\circ X - Y)$ and $M$, where $M:\Omega\rightarrow\{0,1\}$ is a random variable encoding if a specific data record has been used in training of $\targetmodel$ or not.
% The statistic $\hat{M} = 1_{[0.5,1]}\circ m \circ (t\circ X - Y)$ is then used to predict $M$.
% To build the dataset of the membership adversary we take all the testing data of the target which we concatenate with the same number of data records taken from $\mathcal{D}_{train}$.

%This attack is similar to the membership attribute attack described by Yeom et al. \cite{yeom} because it is based on leveraging overfitting. Overfitting is the fact that ML model tends to produce results with more confidence on their training data. This behaviour can be observed numerically by looking a the difference in loss between training and non-training data. In our case the loss used is the difference between the score $t\circ X$ and the label $Y$.

\noindent\textbf{\underline{Metrics.}} \label{sec:metrics} We consider the balanced accuracy %described below
to evaluate the success of AIAs and membership inference attacks.
{Balanced Accuracy} is the average of the proportion of correct predictions of each class of the sensitive attribute individually. 
This is used to account for imbalance in the classes. We refer to balanced accuracy as accuracy in the rest of the paper for brevity. Note that using naive accuracy as an attack metric is misleading when the datasets have significant class imbalance (Table~\ref{tbl:bias}).
Using our previously defined notations, the balanced \aia accuracy is: $\frac{1}{2}(P(\hat{S}=0|S=0) + P(\hat{S}=1|S=1))$.


% \noindent\textbf{\underline{Baselines for Comparison.}}
% \label{sec:baselines} As comparison baselines for the AIA, we use the attacks from Mahajan et al.~\cite{Mahajan2020DoesLS} and Song et al.~\cite{Song2020Overlearning} to evaluate our proposed attacks in threat models \ref{threatmodel2}.
% Both baseline attacks train an attack ML model $\attackmodel$ (also called $a$ in our theory) to map $\targetmodel$'s predictions to different values of the sensitive attribute.
% The Song et al. attack is similar to our \ref{threatmodel2} except that $\upsilon=0.5$ and $\upsilon$ is not optimized in any ways hence loosing the adaptive feature of our attack.
% %, i.e., $\attackmodel: \targetmodel(x) \rightarrow s$. However, they use a default threshold of 0.5 over $\attackmodel$ predictions $\attackmodel(\targetmodel(x))$. If $\attackmodel(\targetmodel(x))$>0.5, then we infer the value of $s \rightarrow$ 1, else $s \rightarrow$ 0. 
% %We use them as baseline attacks to compare with our proposed attacks in both threat models \ref{threatmodel1} and \ref{threatmodel2}.



==> New/misc/new/6eval.tex <==
\section{Evaluation: \adaptiveAIASoft and \adaptiveAIAHard}
\label{sec:evalAIA}


We evaluate the effectiveness of \adaptiveAIASoft and \adaptiveAIAHard in presence of class imbalance for $S(\omega)$ and show the advantage of using an adaptive threshold for soft labels and hard label over the state-of-the-art.


\noindent\textbf{\underline{\adaptiveAIASoft}} When $\targetmodel$ outputs soft labels, we consider the Song et al.~\cite{Song2020Overlearning} and Mahajan et al.~\cite{Mahajan2020DoesLS} as the state-of-the-art baselines to compare against. They use the default $\upsilon=0.5$ over $\attackmodel(\targetmodel(X(\omega)))$ where $\targetmodel(X(\omega))$ are soft labels.


\setlength\tabcolsep{1.5pt}
\begin{table}[!htb]
\caption{Comparing average balanced \aia accuracy over 25 runs for baseline with $\upsilon=0.5$~\cite{Song2020Overlearning,Mahajan2020DoesLS} and \adaptiveAIASoft.}
\label{tab:global_threshold_withoutsattr}
\begin{center}
\footnotesize
\begin{tabular}{ | c | c | c | c | c |  }
\hline
\rowcolor{LightCyan} 
\textbf{Dataset} & \textbf{Baseline ($\upsilon$=0.50)} & \textbf{\adaptiveAIASoft} \\ 
 \rowcolor{LightCyan} & \textbf{\race} | \textbf{\sex} & \textbf{\race} | \textbf{\sex} \\
\hline
\textbf{\census}& 0.50  | 0.53 &\textbf{ 0.58}| \textbf{0.64}\\
\textbf{\compas}& \textbf{0.59} | 0.50 &\textbf{0.59} | \textbf{0.64}\\
\textbf{\meps} & 0.56 | \textbf{0.56} &\textbf{0.59} |\textbf{0.56}\\
\textbf{\law}& 0.61 | \textbf{0.52} &\textbf{0.69} | \textbf{0.52}\\
\textbf{\credit}&0.50 | \textbf{0.55} &\textbf{0.51} | 0.53\\
\hline
\end{tabular}
\end{center}
\end{table}

We present the results in Table~\ref{tab:global_threshold_withoutsattr} for \race and \sex across all the datasets. We see that for the majority of the datasets, \adaptiveAIASoft is atleast as good as or better than the baseline. Hence, \adaptiveAIASoft is an effective \aia compared to prior work.

\noindent\textbf{\underline{\adaptiveAIAHard}} For hard labels, we consider the baseline of training a random forest model as $\attackmodel$ over hard labels to infer the value of $S(\omega)$ for a given $X(\omega)$. We present the effectiveness of \adaptiveAIAHard, fixed threshold over the hard labels, $\targetmodel(X(\omega))$.
We present the comparison of the baseline attack with \adaptiveAIAHard in Table~\ref{tab:global_threshold_withoutsattr_hard}.


\setlength\tabcolsep{1.5pt}
\begin{table}[!htb]
\caption{Comparison of baseline \aia (random forest trained to infer $S(\omega)$ using hard labels from $\targetmodel$ with \adaptiveAIAHard.}
\label{tab:global_threshold_withoutsattr_hard}
\begin{center}
\footnotesize
\begin{tabular}{ | c | c | c | c | c |  }
\hline
\rowcolor{LightCyan}
\textbf{Dataset} & \textbf{Baseline} & \textbf{\adaptiveAIAHard} \\ 
 \rowcolor{LightCyan} & \textbf{\race} | \textbf{\sex} & \textbf{\race} | \textbf{\sex} \\
\hline
\textbf{\census}& 0.50 | 0.50 & \textbf{0.56} | \textbf{0.59} \\ 
\textbf{\compas}& \textbf{0.61} | 0.50 & \textbf{0.61} | \textbf{0.57} \\ 
\textbf{\meps}& \textbf{0.55} | 0.50 & \textbf{0.55} | \textbf{0.52} \\ 
\textbf{\law}& 0.54 | \textbf{0.50} & \textbf{0.54} | \textbf{0.50} \\ 
\textbf{\credit}& 0.50 | \textbf{0.55} & \textbf{0.50} | \textbf{0.55} \\ 
\hline
\end{tabular}
\end{center}
\end{table}

We observe that in all cases, \adaptiveAIAHard is atleast as good as the baseline and in most cases outperforms the baseline. Hence, \adaptiveAIAHard is an effective attack to evaluate against.











\section{Evaluation: Algorithmic Fairness as a Defence}\label{eval:defence}



\subsection{Evaluation: \advdebias}\label{sec:evalDebias}










\subsection{Evaluation: \egddp}
\label{sec:evalEGD}

% correct the threat model

\noindent\textbf{\underline{Effectiveness against \adaptiveAIAHard}} Having shown that our AIA has better performance, we now experimentally illustrate how \egd acts as a defence against attribute inference attack.
We consider two different threat models: \textit{(i)} unprotected setup is when the target model is trained without \egd and the attack is in \ref{threatmodel2}; \textit{(ii)} the defence setup, on the contrary, assumes that the target model has been trained with \egd and the attack is in \ref{threatmodel1}.

\begin{figure}
\subfigure[CENSUS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/CENSUS/race.pdf}}
% \hspace{2mm}
\subfigure[CENSUS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/CENSUS/sex.pdf}}\\
% \hspace{2mm}
\subfigure[COMPAS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/COMPAS/race.pdf}}
% \hspace{2mm}
\subfigure[COMPAS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/COMPAS/sex.pdf}}\\

\subfigure[CREDIT - race]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/CREDIT/race.pdf}}
% \hspace{2mm}
\subfigure[CREDIT - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/CREDIT/sex.pdf}}\\
% \hspace{2mm}
\subfigure[LAW - race]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/LAW/race.pdf}}
% \hspace{2mm}
\subfigure[LAW - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/LAW/sex.pdf}}\\

\subfigure[MEPS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/MEPS/race.pdf}}
% \hspace{2mm}
\subfigure[MEPS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/attack/MEPS/sex.pdf}}
\caption{\egd defence successfully reduces the attack success as predicted by the theory.}
\label{fig:attack}
\end{figure}

We empirically compare the success of the AIA in both the configurations: the unprotected setup and the defence setup.
To do so, we use the five dataset to train a target model with and without the defence.
We use AIA with adaptive threshold to infer the sensitive attribute.
%We repeat this process ten times using cross validation. 

We present the results in Figure~\ref{fig:attack}. We observe that for all datasets the defence successfully reduces the attack success as indicated by the theory. For some datasets, the balanced attack accuracy is slightly above $\frac{1}{2}$; this is due to \egd not reaching perfect demographic parity. In conclusion, we note that \egd is an effective defence against AIA.

\noindent\textbf{\underline{Impact of \egddp on Utility}}
\label{sec:EvalUtility}


\begin{figure}
\subfigure[CENSUS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/CENSUS/race.pdf}}
% \hspace{2mm}
\subfigure[CENSUS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/CENSUS/sex.pdf}}\\
% \hspace{2mm}
\subfigure[COMPAS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/COMPAS/race.pdf}}
% \hspace{2mm}
\subfigure[COMPAS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/COMPAS/sex.pdf}}\\

\subfigure[CREDIT - race]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/CREDIT/race.pdf}}
% \hspace{2mm}
\subfigure[CREDIT - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/CREDIT/sex.pdf}}\\
% \hspace{2mm}
\subfigure[LAW - race]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/LAW/race.pdf}}
% \hspace{2mm}
\subfigure[LAW - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/LAW/sex.pdf}}\\

\subfigure[MEPS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/MEPS/race.pdf}}
% \hspace{2mm}
\subfigure[MEPS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/utility/MEPS/sex.pdf}}
    \caption{On using defence has only a limited impact on the utility.}
    \label{fig:utility}
\end{figure}

We now evaluate how \egd with demographic parity impacts the balanced accuracy of the target model.
We train the target model with and without using \egd and compare the resulting balanced accuracy. 

We present our results across five datasets in Figure~\ref{fig:utility}. For four of the datasets: CENSUS, CREDIT, LAW and MEPS, we do not observe a significant difference in accuracy with an maximum accuracy degradation of ~3\%. For COMPAS dataset, we observe an accuracy degradation of about 7\%. %Depending on the application, this accuracy difference is acceptable. 
In conclusion, using \egd almost does not degrade the balanced accuracy of the target model.




\noindent\textbf{\underline{Computational Overhead}}\label{sec:compcost}

Given the effectiveness of algorithmic fairness as a defence against attribute inference attacks, we ask: \textit{can we get attribute privacy and fairness for free?} We evaluate the computational overhead on using \egd. We train the models for ten iterations with \egd (``Defence'') and without \egd (``Baseline''). We report the mean and standard deviation when in Table~\ref{tab:overhead}. 

\begin{table}[!htb]
\begin{center}
\caption{Training with algorithmic fairness as a defence comes with an additional computational cost during training (indicated in seconds). All the results are over ten runs with p-value$<$0.05.}
\begin{tabular}{ | c | c | c | c | }
\hline
 \rowcolor{LightCyan} \textbf{Dataset} & \textbf{Baseline (s)} & \textbf{Defence (s)} & \textbf{Overhead (\%)}\\ 
 \hline
 \textbf{COMPAS} & 0.27 $\pm$ 0.00 & 15.53 $\pm$ 0.10 & \\  
 \textbf{CENSUS} & 3.29 $\pm$ 0.31 & 138.48 $\pm$ 10.85 & \\  
 \textbf{CREDIT} & 7.30 $\pm$ 0.05 & 726.65 $\pm$ 444.65 & \\  
 \textbf{MEPS} & 1.54 $\pm$ 0.01 & 169.88 $\pm$ 128.80 & \\  
\textbf{LAW} & 0.70 $\pm$ 0.00 & 90.38 $\pm$ 9.20 & \\  
\hline
\end{tabular}
\label{tab:overhead}
\end{center}
\end{table}


We observe that the we get attribute privacy with algorithmic fairness at the cost of computational overhead. We argue that this is still reasonable for a model trainer with basic computational resources (e.g., GPUs). Furthermore, this additional computational cost is incurred naturally if the model trainer is requires to train the model with fairness to meet regulatory requirements~\cite{}. 


\noindent\textbf{\underline{\egd and Membership Inference Attacks}}
\label{sec:EvalMIA}

 
A membership inference attack aims to identify whether a particular target data record was used to train the model. %~\cite{miasurvey}.
Practically, this attack leverages the fact that ML model tends to produce results with more confidence on their $\mathcal{D}_{train}$, especially if the model is overfitted.

\noindent\textbf{Methodology.} Different methodologies have been proposed to conduct a membership inference attack, by looking at the difference in loss between training and non-training data records~\cite{yeom}, or by using one or multiple shadow models~\cite{meminf,carlini2022membership}.
In our case, we consider a methodology similar to Yeom et al.~\cite{yeom} which used the difference of the model loss between the prediction $\targetmodel\circ X$ and ground truth label $Y$.


We train an attack classifier to infer if a data record is a member of the training set of the target model.
This attack classifier is trained on dataset containing the error made by the target model.
Formally, we train the attack classifier $m:[-1,1]\rightarrow[0,1]$ to minimize a mean square error loss on 
$m\circ (t\circ X - Y)$ and $M$, where $M:\Omega\rightarrow\{0,1\}$ is a random variable encoding if a specific data record has been used in training of the target model or not.
The statistic $\hat{M} = 1_{[0.5,1]}\circ m \circ (t\circ X - Y)$ is then used to predict $M$.
To build the dataset of the membership adversary we take all the testing data of the target which we concatenate with the same number of data records taken from $\mathcal{D}_{train}$.



\noindent\textbf{Results.} Chang et al.~\cite{chang2021privacy} show that using \egd with the equality of odds constraint can lead to an increase in the risk of membership inference~\cite{chang2021privacy}.
Here we evaluate the risk of membership inference (as described in Section~\ref{sec:methodoMIA}) of our defence using demographic parity as fairness constraint.
Figure~\ref{fig:mia} reports for all datasets and for both \race and \sex attributes, this risk of membership inference for our defence and for a target model without fairness regularization.
Results show that for four datasets over five, the overall privacy risk to membership inference is not impacted. For CREDIT dataset, we observe a decrease in the overall risk to membership inference attack for our defence. 
% Hence, unlike Chang et al.~\cite{chang2021privacy}, we note that using demographic parity does not increase the risk to membership inference attacks.


%We present our results in Figure~\ref{fig:mia} for different datasets for both \race and \sex attributes. We note that in four of the dataset, the overall privacy risk to membership inference is not impacted. For CREDIT dataset, we observe a decrease in the overall risk to membership inference attack. Hence, unlike Chang et al.~\cite{chang2021privacy}, we note that using demographic parity does not exacerbate the risk to membership inference attacks.


%Our defence uses demographic parity as fairness constraint but we still evaluate the impact on membership inference risk.

%We evaluate the risk to membership inference using the five dataset presented in Section~\ref{sec:datasets}.
%We train the target model once without using \egd and once using \egd.
%We then run the membership inference attack described in Section~\ref{sec:methodoMIA}. We repeat this process ten times with cross validation.

\begin{figure}
\subfigure[CENSUS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/CENSUS/race.pdf}}
% \hspace{2mm}
\subfigure[CENSUS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/CENSUS/sex.pdf}}\\
% \hspace{2mm}
\subfigure[COMPAS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/COMPAS/race.pdf}}
% \hspace{2mm}
\subfigure[COMPAS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/COMPAS/sex.pdf}}\\

\subfigure[CREDIT - race]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/CREDIT/race.pdf}}
% \hspace{2mm}
\subfigure[CREDIT - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/CREDIT/sex.pdf}}\\
% \hspace{2mm}
\subfigure[LAW - race]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/LAW/race.pdf}}
% \hspace{2mm}
\subfigure[LAW - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/LAW/sex.pdf}}\\

\subfigure[MEPS - race]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/MEPS/race.pdf}}
% \hspace{2mm}
\subfigure[MEPS - sex]{\includegraphics[width=0.22\textwidth]{image/annexe/mia/MEPS/sex.pdf}}
    \caption{Fairness regularization using \egd based on demographic impact does not increase the risk of membership inference.
    }
    %\caption{Impact of \egd for fair classification on membership inference attack. Except for CREDIT where it seems that the fairness algorithm has decreased the success of the attack,    there is no real impact on membership leakage.}
    \label{fig:mia}
\end{figure}





%We present our results in Figure~\ref{fig:mia} for different datasets for both \race and \sex attributes. We note that in four of the dataset, the overall privacy risk to membership inference is not impacted. For CREDIT dataset, we observe a decrease in the overall risk to membership inference attack. Hence, unlike Chang et al.~\cite{chang2021privacy}, we note that using demographic parity does not exacerbate the risk to membership inference attacks.

% \noindent\textbf{Comparison with Chang et al.~\cite{chang2021privacy}}Finally, we try to comfort the observations described by Chang et al.~\cite{chang2021privacy} (i.e., \egd with the equality of odds constraint can lead to increase the risk of membership inference). To achieve that, we train $\targetmodel$ with \egd using equality of odds as a fairness constraint. We then evaluate the risk of membership inference.
% Figure\ref{fig:miaeoo} depicts this risk.
% Although the implementation of the MIA is slightly different, we do not observe an amplification of the membership inference as shown by Chang et al. \cite{chang2021privacy}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.60\linewidth]{image/miaeoo.pdf}
%     \caption{\egd based on equality of odds constraint does not increase the risk of membership inference in our setting (Law dataset, Race attribute).}
%     \label{fig:miaeoo}
% \end{figure}


\subsection*{Impact of Other Factors on \egddp}
\label{sec:otherfactors}

We now perform a study of different hyperparameters and configurations which can impact the success of \egd defence: model architecture (Section~\ref{sec:archi}), shift in the distribution between \adv's $\mathcal{D}_{aux}$ and target model's $\mathcal{D}_{train}$ (Section~\ref{sec:Advknowledge}), changing the fairness constraint (Section~\ref{sec:eoolimit}), and comparison with using hard label's information bottleneck (Section~\ref{sec:hardlabel}).\\

\noindent\textbf{\underline{Impact of model architecture}}
\label{sec:archi}
Theorem \ref{th:dpgood} is independent of any specific architecture of the target model (i.e., the underlying expression of $\targetmodel$).
We evaluate \egd defence on two types of architecture of the target model.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\linewidth]{image/rfvsnn.pdf}
    \caption{We do not observe a decrease in effectiveness of the defence when the target model uses a perceptron compared to random forest.}
    \label{fig:rfvsnn}
\end{figure}

We present the results in Figure~\ref{fig:rfvsnn} for LAW (\race) by comparing the balanced attack accuracy when the target model is a random forest and a perceptron. A perceptron is a binary classifier, its architecture is the same as a neural network with one layer.
%On comparing the attack success of the two architectures of target models, random forest (left) and MLP (right), 
Results show that there is no significant decrease in the defence on using a perceptron by comparison with a random forest.\\


\noindent\textbf{\underline{Impact of \adv's Knowledge}}
\label{sec:Advknowledge}

\adv uses $\mathcal{D}_{aux}$ to train an attack model inferring the value of sensitive attribute from the model prediction.
The distribution of this auxiliary dataset has an impact on the attack accuracy. Previously, we assumed that \adv has a dataset sampled from the same distribution as the target model's $\mathcal{D}_{train}$. The theoretical guarantees in Theorem~\ref{th:dpgood} is based on this assumption. However, this is not always a realistic scenario.

%Indeed in the proof we have used $P=Q$, $P$ begin the distribution of the target's model dataset and $Q$ the one for $\mathcal{D}_{aux}$.
%We cannot prove theorem \ref{th:dpgood} without a relation between $P$ and $Q$ because the balanced attack accuracy is computed under $Q$ and the demographic parity is true under $P$.



%In this experiment we assume that the data's distribution of $\mathcal{D}_{aux}$ is the same as the data's distribution of the target model : it might not always be the case in realistic scenarios.
%This assumption is needed to have the full theoretical guarantees of theorem \ref{th:dpgood}.
%Indeed in the proof we have used $P=Q$, $P$ begin the distribution of the target's model dataset and $Q$ the one for $\mathcal{D}_{aux}$.
%We cannot prove theorem \ref{th:dpgood} without a relation between $P$ and $Q$ because the balanced attack accuracy is computed under $Q$ and the demographic parity is true under $P$.

We experimentally evaluate the impact of distribution shift between the auxiliary and target model's $\mathcal{D}_{train}$ on the AIA and on the defence. We use the Retiring Adult dataset~\cite{folk} which is a wrapper around the CENSUS dataset and makes it easy to select the U.S. state to sample the dataset from.
Since the demographics change from one state to another, training the target model on one state and the attack on another allows to test the influence of realistic statistical disparities.
We use data records from the state of New York to train the target model. We perform AIA by sampling different datasets of different states as auxiliary dataset.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\linewidth]{image/BaVsState.pdf}
    \caption{The more the data used to train the target model are different from those used to train the attack, the lower the accuracy tends to be, however the effectiveness of the defence using fairness regularization is not affected.
    }
    \label{fig:shift}
        %An auxiliary knowledge which does not respect the statistical distribution of the dataset used for training the target model reduces the success of the attack. 
\end{figure}

As a metric to capture the difference in distribution, we use the distribution shift score from the Synthetic Data Vault framework~\cite{SDV}.
This score combines multiple standard ways to evaluate the shift in distribution between two datasets into a score indicating how alike two datasets are.

We present the results in Figure~\ref{fig:shift} which depicts the attack accuracy according to the distribution shift when the target model is trained with and without fairness regularization as a defence.

Firstly, using the same data to train both the target model and \adv model provides an upper bound of the attack accuracy.
When the data used to train the target model is different from \adv's auxiliary data, the attack accuracy decreases.
However, we also show that the distribution shift does not affect the performance of the defence. Specifically, in every case the defence using the fairness regularization limits the attack accuracy close to a random guess (i.e., an accuracy at $0.5$).\\








\noindent\textbf{\underline{Impact of Using Hard Labels}}
\label{sec:hardlabel}

Instead of providing a prediction in the form of a soft label (i.e., a score between 0 and 1), $\targetmodel$ can binarized the model prediction. In this case, \adv can only observe this binarized prediction to conduct its AIA.
This threat model is similar to \ref{threatmodel2} except that \adv has access to a collection of $\hat{Y}(\omega_0),\cdots,\hat{Y}(\omega_{A-1})$ records to attack.
$\hat{Y}$ is often called \textit{hard label}.
In this case, $\mathcal{D}_{aux}$ comes from the distribution $Q_{\hat{Y},S}$ and the attack model is $a:\{0,1\}\rightarrow[0,1]$.
The attacker can then build a statistic $\hat{S}$ to infer $S$:
\begin{equation}
    \label{eq:hardtm}
    \hat{S}=1_{[\upsilon,1]}\circ a\circ \hat{Y}\circ X,
\end{equation}
where $\upsilon \in [0,1]$ is a threshold that can be learned to account for class imbalance.
This threat model makes the attack harder to perform in comparison with \ref{threatmodel2} because oftentimes $\hat{Y}=1_{[\tau,1]}\circ \targetmodel\circ X$.
In this expression, we see that in comparison with equation \ref{eq:tm1}, equation \ref{eq:hardtm} adds a bottleneck with the indicator function doing the threshold.
In this section we realize an empirical evaluation of the impact of this bottleneck of information.


%In \ref{threatmodel2}, \adv has access to hard labels (a binary vector indicating 1 for correct class label and 0 for all the remaining classes) to perform the attack. 
%We now evaluate the effectiveness of using hard labels instead of soft labels. The intuition is that using hard labels will minimize the amount of information available to \adv making the effectiveness of the attack lower. To validate this intuition, we obtain hard labels from the soft prediction scores by applying the argmax function over the prediction scores. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\linewidth]{image/hardvsdef.pdf}
    \caption{Using hard labels (i.e., binarized prediction) can reduce the accuracy of an AIA but is less efficient than a fairness regularization using demographic impact.} 
    \label{fig:hardvsdef}
\end{figure}

Figure~\ref{fig:hardvsdef} compares the attack accuracy for LAW dataset (\race) of a $\targetmodel$ using hard labels against a $\targetmodel$ using soft label (i.e., \ref{threatmodel2} referred as ``baseline'' in Figure~\ref{fig:hardvsdef}), and a $\targetmodel$ using fairness regulation based on demographic impact (i.e., \ref{threatmodel1}).
Results show that the balanced attack accuracy for hard labels is lower on average than for the soft labels. 
Indeed, hard labels acts as a bottleneck of information by reducing the attack success in comparison with soft labels. However, \egd defence is more efficient by limiting the attack accuracy close to random guess (i.e., an accuracy at 0.5) thanks to theoretical guarantees.

%We present the results for LAW dataset (\race) in Figure~\ref{fig:hardvsdef} to evaluate the impact of using hard labels and compare it with baseline attack accuracy and on using our \egd defence. We note that the balanced attack accuracy is lower on average than the baseline attack accuracy. This validates our intuition that using hard labels indeed reduces the overall risk to AIAs. The use of hard labels acts as a bottleneck of information by reducing the attack success in comparison with \ref{threatmodel2} (``baseline'' in Figure~\ref{fig:hardvsdef}). However, we note that despite using hard label it is possible to infer the value of sensitive attributes as seen in the boxplot.

%Clearly, using \egd reduces the risk much more effectively than using hard labels. Furthermore, using hard labels does not provide any theoretical guarantees on the reduction of risk to AIAs.






==> New/misc/new/7discussions.tex <==
\section{Discussions}
\label{sec:discussions}


We first empirically validate the theoretical result (Theorem~\ref{th:eoo}) of lower success of \eo to mitigate AIAs (Section~\ref{sec:eoolimit}). We evaluate the influence of this fair classification strategy on the success of membership inference attacks to get a full picture of \egd on privacy (Section~\ref{sec:EvalMIA}).


\noindent\textbf{\underline{Ineffectiveness of \egdeo.}} In Theorem~\ref{th:dpgood} and Theorem~\ref{th:eoo}, we theoretically show that \demparity provides better guaranties than \eo to lower the distinguishability and thereby attack success to attribute inference attack. We want to validate this experimentally by showing that equality odds is less effective as a defence against an AIA than \demparity.


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{image/dpvseoo.pdf}
    \caption{Fairness regularization based on \eo provides less guaranty against an AIA than a regularization based on demographic impact (LAW dataset, \race attribute).}
    \label{fig:dovseoo}
\end{figure}

For experimental evaluation, we train models on LAW dataset (\race) using \demparity and \eo. We present the results in Figure~\ref{fig:dovseoo}. We note that the average attack accuracy for \demparity is lower than \eo. Hence, our experimental evaluation validates our theoretical results. This also supports our reasoning for choosing \demparity over \eo.



\noindent\textbf{\underline{Generalization to High Dimensional Data}} To demonstrate the generalization of our defense to high dimensional data, we report the results on the LFW dataset, an image datasets with 2914 attributes per data record. We use a fully connected neural network with 4 layers as target model. Our defense comforts other results by reducing the inference of \sex attribute from  0.65 $\pm$ 0.10 to  0.50 $\pm$ 0.00. 

==> New/misc/new/8related.tex <==
\section{Related Work}
\label{sec:related}

\noindent\textbf{\aia{s}} have been extensively studied in the context of online social media where \adv can leverage user's behavioural information~\cite{attinfSocial1,attinfSocial2,attinfSocial3,attinfSocial4,attinfSocial5,attinfSocial6}. In ML, \aia{s} are approached as data imputation challenges~\cite{fredrikson2,yeom,MehnazAttInf} and by leveraging intermediate model representations~\cite{Song2020Overlearning,Mahajan2020DoesLS,malekzadeh2021honestbutcurious}, which we extensively cover in Section~\ref{sec:back-attribute}.

Moreover, \adv can execute \aia using \mia as a subroutine~\cite{yeom}. The success of \aia{s} mirrors that of \mia{s}, hinging on the degree of $\targetmodel$ overfitting. Nevertheless, Zhao et al.\cite{memprivNattpriv} establish this link only holds when \mia{s} are highly effective. If not, \aia{s} offer minimal advantage, despite the model's vulnerability to \mia{s}. Additionally, \aia{s} are effective against model explanations, presenting a compromise between attribute privacy and transparency~\cite{duddu2022inferring}.



% TODO ADD: \cite{Malekzadeh_2021}


\noindent\textbf{Mitigating \aia{s}} has limited prior literature. Attriguard~\cite{attriguard} safeguards sensitive attributes in social networks by introducing adversarial noise to the output predictions, compelling $\attackmodel$ to make incorrect classifications. In the realm of ML, adversarial training has proven effective in diminishing the identifiability of sensitive attributes within predictions~\cite{NEURIPS2020_6b8b8e3b}. This technique can additionally disentangle sensitive features from model representations~\cite{10.5555/3122009.3208010,10.5555/3327546.3327583,10.5555/3294771.3294827,pmlr-v80-madras18a,censoringadv}. An alternative avenue, variational autoencoders, was explored for minimizing \aia{s}\cite{10.5555/3042817.3042973}; however, Song et al.\cite{Song2020Overlearning} found these defences to be ineffective.

\noindent\textbf{Interactions between Privacy and Fairness} have been explored in prior work~\cite{chang2021privacy,indivfairness,dpaccdisp,dpfair,fioretto2022differential,pate2021fairness}. Chang et al.~\cite{chang2021privacy} demonstrate that applying in-processing fairness algorithms escalates overfitting, heightening vulnerability to \mia{s}, particularly affecting minority subgroups. Additionally, differential privacy and individual fairness share a common goal, with individual fairness encompassing differential privacy as a broader concept~\cite{indivfairness}. However, differential privacy and group fairness are at odds when there's performance discrepancy between minority and majority subgroups~\cite{dpaccdisp,dpfair,fioretto2022differential,pate2021fairness}. Ferry et al.~\cite{10136153} introduced \aia aimed at predicting sensitive attributes from a fair model. Their approach assumes that the fairness algorithm used in model training is known to \adv, enabling calibration of the attacks. However, in practice, revealing model training specifics for confidentiality is improbable. In distinction from their approach, our attacks function within the context of \adv's blackbox understanding of $\targetmodel$, and the defenses we present effectively counter such attacks.




==> New/misc/new/9conclusions.tex <==
\section{Conclusions and Future Work}\label{sec:conclusions}
 
\noindent\textbf{\underline{Summary of Contributions.}} We demonstrate the alignment of algorithmic group fairness and attribute privacy, crucial components for building trust in machine learning (ML). This reveals that training a model with algorithmic fairness can simultaneously offer attribute privacy against a blackbox \adv. We examine two scenarios where \adv obtains either soft or hard labels from $\targetmodel$, and we introduce improved \aia{s}: \adaptiveAIASoft and \adaptiveAIAHard.

Regarding \adaptiveAIASoft, we establish that \advdebias serves as a potent defense mechanism. It achieves fairness by ensuring indistinguishable predictions while accounting for a potential \adv during training. For \adaptiveAIAHard, we propose \egd with established fairness constraints: \demparity and \eo. Our theoretical and empirical analysis substantiates that \egddp is the optimal defense strategy against any \aia.


\noindent\textbf{\underline{Limitations and Future Work.}} We enhance existing \aia{s} and introduce two attacks for $\targetmodel$'s outputs: soft labels (\adaptiveAIASoft) and hard labels (\adaptiveAIAHard). Our advancements surpass previous \aia{s}, although their optimality remains uncertain under the assumption of a powerful \adv with any possible background knowledge. As part of our future research, we are investigating the development of an optimal attack in this context. Moreover, creating a defense against an optimal \aia could assist in evaluating the optimality of current defenses and guide the formulation of more principled defenses.

